HARP-Net: Hedging-Aware Refinement Pricing Network for Option Pricing

Dynamic option hedging requires a pricing function whose local sensitivities remain reliable throughout complete hedge-to-expiry paths. However, most neural option pricing models are trained as pointwise price predictors, so their induced hedge ratios are only indirectly connected to realized replication performance. We propose the Hedging-Aware Refinement Pricing Network (HARP-Net), a neural option pricing framework that learns an explicit and differentiable pricing surface while directly aligning optimization with pathwise hedging outcomes. HARP-Net combines four components: \emph{(i)} a temporal encoder that summarizes rolling option-state dynamics, \emph{(ii)} domain-wise embeddings that preserve the distinct financial roles of heterogeneous state variables, \emph{(iii)} a bounded residual anchor that stabilizes the initial latent pricing state, and \emph{(iv)} a gated bridge-refinement mechanism that applies controlled context-dependent corrections. The final pricing surface is differentiated with respect to the underlying asset to obtain the model-implied delta, and the network is trained using squared self-financing hedging PnL rather than relying solely on price-regression supervision. We evaluate HARP-Net on four DJX and XEO call and put datasets against analytical, machine-learning, and deep-learning baselines. The results show that HARP-Net achieves the strongest overall hedging performance across the reported assessment metrics while maintaining a favorable balance between computational cost and predictive capabilities.

==> algorithms/hedge_loss_training.tex <==
\begin{algorithm}[!htbp]
\caption{Pathwise Delta Hedge-Loss Training}
\label{alg:hedge_loss_training}
\small

\setlength{\abovedisplayskip}{4pt}
\setlength{\belowdisplayskip}{4pt}

\begin{algorithmic}[1]

\Require Training paths $\mathcal{D}_{\mathrm{train}}$,
validation paths $\mathcal{D}_{\mathrm{val}}$,
pricing model $f_\theta$, learning rate $\eta$,
path-batch size $B$, maximum epochs $E$,
early-stopping patience $p_{\mathrm{stop}}$.

\Ensure Validation-selected parameters $\theta^\star$.

\State Initialize Adam with learning rate $\eta$.
\State Initialize the best validation loss to $+\infty$.

\For{$e=1,\ldots,E$}

    \State Set the model to training mode.

    \State Partition $\mathcal{D}_{\mathrm{train}}$
    into path mini-batches $\{\mathcal{B}_j\}$.

    \For{each mini-batch $\mathcal{B}_j$}

        \State Clear accumulated parameter gradients.

        \For{each path $p\in\mathcal{B}_j$}

            \State Evaluate $P_\theta(p)$ using
            Algorithm~\ref{alg:pathwise_evaluation},
            retaining the autograd graph.

        \EndFor

        \State Compute the batch loss:
        \[
        \mathcal{L}_j=
        \frac{1}{|\mathcal{B}_j|}
        \sum_{p\in\mathcal{B}_j}P_\theta(p)^2.
        \]

        \State Backpropagate $\mathcal{L}_j$.
        \State Clip the parameter-gradient norm to $5$.
        \State Update $\theta$ using Adam.

    \EndFor

    \State Set the model to evaluation mode.

    \State Evaluate validation paths using autograd
    without retaining higher-order training graphs.

    \State Compute the validation loss:
    \[
    \mathcal{L}_{\mathrm{val}}=
    \frac{1}{|\mathcal{D}_{\mathrm{val}}|}
    \sum_{p\in\mathcal{D}_{\mathrm{val}}}P_\theta(p)^2.
    \]

    \State Save $\theta$ as $\theta^\star$
    if validation loss improves.

    \State Stop if validation loss does not improve
    for $p_{\mathrm{stop}}$ consecutive epochs.

\EndFor

\State Restore and \Return $\theta^\star$.

\end{algorithmic}
\end{algorithm}

==> algorithms/pathwise_evaluation.tex <==
\begin{algorithm}[!htbp]
\caption{Pathwise Delta-Hedging PnL Evaluation}
\label{alg:pathwise_evaluation}
\small

\setlength{\abovedisplayskip}{4pt}
\setlength{\belowdisplayskip}{4pt}

\begin{algorithmic}[1]

\Require Complete option path $p$, pricing model $f_\theta$,
option style $a\in\{C,P\}$, train-fitted scalers.

\Ensure Terminal hedging PnL $P_\theta(p)$.

\State Let $\ell_t=\log(S_t/K)$ and let $s_y$, $s_\ell$
denote the inverse MinMax scaling coefficients.

\State Compute the model-implied delta at each live observation:
\[
\widehat{\Delta}_t
=
\frac{s_y}{s_\ell S_t}
\frac{
\partial f_\theta(\widetilde{x}_{t,\mathrm{seq}})
}{
\partial\widetilde{\ell}_t
}.
\]

\State Define the terminal payoff:
\[
\Phi_a(S_T^\star,K)=
\begin{cases}
\max(S_T^\star-K,0), & a=C,\\
\max(K-S_T^\star,0), & a=P.
\end{cases}
\]

\State Initialize the underlying holding and cash account:
\[
h_0=\widehat{\Delta}_0,
\qquad
c_0=V_0^{\mathrm{obs}}-h_0S_0.
\]

\For{$t=1,\ldots,T-1$}

    \State Accrue interest and dividend income:
    \[
    c_t^- =
    c_{t-1}e^{r_{t-1}\Delta t_t}
    +h_{t-1}S_{t-1}q_{t-1}\Delta t_t.
    \]

    \State Rebalance the underlying position:
    \[
    \begin{aligned}
    c_t &= c_t^-
    -(\widehat{\Delta}_t-h_{t-1})S_t,\\
    h_t &= \widehat{\Delta}_t.
    \end{aligned}
    \]

\EndFor

\State Accrue the final holding interval:
\[
c_T^- =
c_{T-1}e^{r_{T-1}\Delta t_T}
+h_{T-1}S_{T-1}q_{T-1}\Delta t_T.
\]

\State Compute terminal hedging PnL:
\[
P_\theta(p)=
c_T^-+h_{T-1}S_T^\star-\Phi_a(S_T^\star,K).
\]

\State \Return $P_\theta(p)$.

\end{algorithmic}
\end{algorithm}

==> sections/04_experiments/comparative_models.tex <==

\subsection{Comparative Models}
\label{subsec:comparative_models}

To evaluate the effectiveness of HARP-Net, we consider
a diverse set of comparative models comprising five
classical and numerical option pricing methods and
fourteen neural architectures. The selected models
represent different approaches to financial modelling
and sequential representation learning, including
analytical pricing, numerical approximation, feedforward
networks, recurrent networks, convolutional architectures,
linear time-series models, and attention-based methods.

\paragraph{Classical and numerical pricing models.}

\begin{itemize}

    \item \textbf{Black--Scholes (BS):}
    The Black--Scholes model \cite{black1973pricing}
    provides a closed-form solution for European
    option prices under the assumption that the
    underlying asset follows a geometric Brownian
    motion with constant volatility. Its analytical
    delta provides a fundamental benchmark for
    evaluating the dynamic hedging performance of
    the proposed framework.

    \item \textbf{Merton Jump-Diffusion Model:}
    The Merton model \cite{merton1976option}
    extends the Black--Scholes framework by incorporating
    discontinuous changes in the underlying asset price
    through a compound Poisson jump process. Option
    prices and hedge sensitivities are calculated using
    a truncated Poisson-weighted series of
    Black--Scholes quantities. This model provides a
    benchmark for assessing the effect of incorporating
    discontinuous price movements into the pricing
    dynamics.

    \item \textbf{Heston Model:}
    The Heston model \cite{heston1993closed}
    introduces stochastic volatility by modelling the
    instantaneous variance of the underlying asset
    through a mean-reverting square-root diffusion
    process. Option prices are evaluated using numerical
    integration of the characteristic-function-based
    pricing representation, while hedge sensitivities
    are estimated through finite-difference
    perturbations.

    \item \textbf{Binomial Tree:}
    The Cox--Ross--Rubinstein binomial model
    \cite{cox1979option} approximates the evolution of
    the underlying asset through a recombining
    discrete-time tree. Option prices are obtained
    by backward induction from the terminal payoff
    using risk-neutral transition probabilities.
    The model provides a discrete-time numerical
    counterpart to continuous-time option pricing
    frameworks.

    \item \textbf{Finite Difference Method (FDM):}
    The finite difference method numerically solves
    the Black--Scholes partial differential equation
    by discretizing the underlying-price and time
    domains. The adopted implementation uses an
    implicit Euler time-stepping scheme and solves
    the resulting tridiagonal linear systems.
    Option prices are obtained by interpolation
    over the numerical price grid, and hedge
    sensitivities are estimated using finite
    differences.

\end{itemize}

\paragraph{Feedforward and recurrent neural models.}

\begin{itemize}

    \item \textbf{Multilayer Perceptron (MLP):}
    Feedforward neural networks provide a
    nonparametric approach to option pricing
    \cite{hutchinson1994nonparametric}.
    In the adopted implementation, the rolling
    option-state window is flattened into a
    one-dimensional feature vector and passed
    through fully connected layers with nonlinear
    activations. A scalar output layer produces
    the normalized option price.

    \item \textbf{Long Short-Term Memory (LSTM):}
    LSTM \cite{hochreiter1997long} is a recurrent
    neural architecture that uses gated memory
    cells to capture temporal dependencies.
    The model processes the rolling option-state
    sequence, and its final recurrent representation
    is mapped to a scalar option price. It provides
    a benchmark for evaluating the contribution of
    recurrent temporal modelling.

    \item \textbf{Gated Recurrent Unit (GRU):}
    GRU \cite{chung2014empirical} employs update
    and reset gates to control the propagation of
    historical information through recurrent hidden
    states. Compared with LSTM, it uses a simpler
    gating structure. The terminal hidden state
    of the GRU encoder is passed through a
    feedforward pricing head.

    \item \textbf{DeepAR:}
    DeepAR \cite{salinas2020deepar} is a recurrent
    probabilistic forecasting architecture that
    parameterizes a predictive distribution using
    an autoregressive neural representation.
    In this study, its recurrent encoder produces
    distributional parameters, with the predicted
    mean serving as the deterministic option
    price output. The hedge-loss objective is
    applied to the sensitivities derived from
    this mean prediction.

\end{itemize}

\paragraph{Convolutional and hybrid neural models.}

\begin{itemize}

    \item \textbf{One-Dimensional Convolutional
    Neural Network (CNN1D):}
    CNN1D extracts local temporal patterns by
    applying one-dimensional convolutional filters
    across successive option-state observations.
    The resulting feature maps are aggregated
    using global average pooling and transformed
    into a scalar option price through a linear
    output layer.

    \item \textbf{Residual Network (ResNet):}
    ResNet employs residual connections to
    facilitate the propagation of information
    through stacked convolutional blocks.
    The adopted one-dimensional architecture
    extracts temporal representations using
    residual convolutional layers, followed by
    global average pooling and a feedforward
    pricing head.

    \item \textbf{CNN-LSTM:}
    CNN-LSTM combines convolutional feature
    extraction with recurrent temporal modelling.
    The convolutional layers first extract local
    patterns from the option-state sequence.
    These representations are subsequently
    processed by an LSTM encoder, whose hidden
    representation is mapped to the option price.

    \item \textbf{CNN-BiLSTM:}
    CNN-BiLSTM extends the convolutional-recurrent
    architecture by incorporating a bidirectional
    LSTM encoder. The forward and backward hidden
    representations are concatenated before the
    scalar pricing head. Both recurrent directions
    operate exclusively within the historical
    lookback window, without accessing observations
    beyond the current valuation time.

\end{itemize}

\paragraph{Linear time-series models.}

\begin{itemize}

    \item \textbf{DLinear:}
    DLinear \cite{zeng2023transformers} decomposes
    an input time series into trend and residual
    components using a moving-average operation.
    Separate linear transformations are applied
    to the two components, and their outputs
    are subsequently combined. In the adopted
    implementation, a channel-mixing network
    aggregates the resulting feature-wise
    representations into a scalar option price.

    \item \textbf{NLinear:}
    NLinear \cite{zeng2023transformers} reduces
    sensitivity to temporal level shifts by
    subtracting the final observation from each
    input feature before applying a linear
    temporal transformation. The removed value
    is subsequently restored, and the resulting
    feature-wise outputs are combined through
    a channel-mixing network to produce the
    normalized option price.

\end{itemize}

\paragraph{Attention-based and advanced time-series models.}

\begin{itemize}

    \item \textbf{Transformer:}
    The Transformer architecture
    \cite{vaswani2017attention} employs multi-head
    self-attention to model interactions between
    observations within an input sequence.
    The option-state features are projected into
    a latent embedding space and augmented with
    positional encodings. The resulting sequence
    is processed by Transformer encoder layers,
    and the final temporal representation is
    mapped to a scalar option price.

    \item \textbf{Patch Attention (PAttn):}
    PAttn partitions the input time series into
    overlapping temporal patches and transforms
    them into patch-level representations.
    Self-attention is applied across these
    representations to capture temporal
    dependencies at the patch level. The
    resulting feature forecasts are subsequently
    mapped to an option price through a
    feedforward pricing head.

    \item \textbf{TimeXer:}
    TimeXer \cite{wang2024timexer} is a Transformer-based
    time-series architecture designed to model
    temporal dependencies and interactions
    between endogenous and exogenous variables.
    Its attention-based representations capture
    relationships among the input feature
    sequences. The resulting multivariate output
    is transformed into a scalar option price
    using a feedforward pricing head.

    \item \textbf{WPMixer:}
    WPMixer \cite{murad2025wpmixer} is a time-series
    forecasting architecture based on temporal
    patching and feature-mixing operations.
    Although the original architecture supports
    wavelet-based multiresolution decomposition,
    the configuration evaluated in this study
    disables the wavelet decomposition stage.
    The resulting backbone outputs are mapped
    to a scalar option price through a
    feedforward pricing head.

\end{itemize}

\paragraph{Adaptation to a common hedging framework.}

To ensure a consistent comparison, all neural models
are formulated as scalar option pricing functions
operating on the same normalized rolling option-state
window,
\begin{equation}
    f_{\theta}^{(m)}:
    \mathbb{R}^{L\times D}
    \rightarrow
    \mathbb{R},
    \label{eq:comparative_pricing_map}
\end{equation}
where $m$ denotes the comparative model, $L$ is the
lookback length, and $D$ is the number of input
features.

For a normalized input sequence
$\widetilde{\mathbf{X}}_t$, the corresponding
normalized scalar output is given by
\begin{equation}
    \widehat{y}_t^{(m)}
    =
    f_{\theta}^{(m)}
    \left(
        \widetilde{\mathbf{X}}_t
    \right).
    \label{eq:comparative_model_output}
\end{equation}

For architectures originally developed for
multivariate time-series forecasting, an additional
pricing head transforms the backbone representation
into a scalar option price. Although these
architectures employ internal forecasting operations,
their final pricing outputs correspond to the current
valuation time rather than a future option price.

The model-implied hedge ratios are obtained by
differentiating the resulting pricing functions
with respect to the current underlying level,
following the procedure described in
Section~\ref{subsec:hedging_training}.

All neural models, including HARP-Net, are trained
using the same pathwise squared hedging PnL objective.
Consequently, the primary neural comparison evaluates
differences in architectural representation under
a common hedging-aware optimization framework,
rather than differences arising from independently
selected training objectives.

The classical and numerical models obtain hedge
sensitivities from their corresponding pricing
functions through analytical differentiation or
finite-difference approximation. All comparative
models are evaluated on identical test paths using
the same self-financing portfolio accounting and
terminal settlement conventions. Model-specific
configurations and training procedures are described
in Section~\ref{subsec:experimental_setup}.


==> sections/04_experiments/data_description.tex <==
\subsection{Data Description}
\label{subsec:data_description}

The experimental analysis uses historical option data
obtained from iVolatility.com for two underlying indices:
the Dow Jones Industrial Average (DJX) and the S\&P 100
Index (XEO). The original datasets contain daily
observations from November 2, 2020, to October 31, 2025,
comprising 1,187,848 observations across 13,468 distinct
DJX option contracts and 2,323,593 observations across
27,960 distinct XEO option contracts. Both datasets
contain European-style call and put options, which are
considered separately, resulting in four experimental
datasets: DJX-Call, DJX-Put, XEO-Call, and XEO-Put.

Each observation contains contract-specific and
market-specific information, including the observation
date, option identifier, expiration date, strike price,
underlying index level, bid and ask quotes, option price,
implied volatility, trading volume, and open interest.
The datasets also contain option sensitivities, namely
delta, gamma, vega, theta, and rho. The underlying index
levels, strike prices, and option premiums are expressed
in index points, while implied volatility is represented
in decimal form.

In addition to the option data, daily U.S. Treasury
par yield curve data are used to obtain maturity-dependent
risk-free interest rates. The Treasury yield data provide
interest rates across multiple maturities, allowing the
financing rate associated with each option observation
to reflect its remaining time to expiration.

Following the contract selection procedures described
in Section~\ref{subsec:data_preprocessing}, the
experimental datasets contain 45,322 DJX observations
across 1,021 distinct contracts and 261,330 XEO
observations across 7,820 distinct contracts.
The retained observations span November 2021 to
October 2025. Table~\ref{tab:dataset_spec} summarizes
the number of observations, distinct contracts, and
their initial moneyness classifications for each
experimental dataset.

\input{tables/experimental_setup}

==> sections/04_experiments/data_preprocessing.tex <==

\subsection{Data Preprocessing}
\label{subsec:data_preprocessing}

An essential requirement for evaluating dynamic option
hedging is the construction of temporally consistent
contract paths that preserve the evolution of market
variables from hedge initiation to expiration.
Unlike conventional option pricing studies that treat
individual observations as independent samples, our
preprocessing procedure retains the sequential structure
of each option contract. The procedure consists of data
cleaning, contract selection, financial feature
construction, rolling window generation, chronological
partitioning, and normalization.

\paragraph{Data cleaning and contract selection.}

The observation and expiration dates are first converted
to a consistent datetime format, while the underlying
index level, strike price, option premium, and implied
volatility are converted to numerical values.
Observations with invalid dates, non-positive underlying
levels or strike prices, and negative time to expiration
are excluded. For observations preceding expiration,
the option premium and implied volatility are required
to be finite and strictly positive. Terminal observations
are treated separately because the option premium may
be zero and implied volatility may be undefined at
expiration.

Each option contract is identified using the combination
of its underlying symbol, exchange, and option identifier.
The observations are grouped by contract and sorted
chronologically. Call and put contracts are processed
separately.

To establish comparable hedge-initiation conditions,
contracts are selected using their moneyness and remaining
days to expiration. Let
\begin{equation}
    M_t = \frac{S_t}{K}
    \label{eq:option_moneyness}
\end{equation}
denote the moneyness of an option at observation $t$,
where $S_t$ is the underlying index level and $K$ is
the strike price. Let $D_t$ denote the number of calendar
days between the observation date and the expiration date.

A contract is eligible for hedge initiation at observation
$t$ if
\begin{equation}
    0.96 \leq M_t \leq 1.04,
    \qquad
    3 \leq D_t \leq 45.
    \label{eq:initiation_conditions}
\end{equation}

In addition, the contract must contain sufficient
historical observations to construct a rolling input
window of length $L$. Let
$\{t_1,t_2,\ldots,t_n\}$ denote the chronologically
ordered observation dates of a contract. The
hedge-initiation index is defined as
\begin{equation}
    i_0 =
    \min \left\{
        i \geq L :
        0.96 \leq M_{t_i} \leq 1.04,\;
        3 \leq D_{t_i} \leq 45
    \right\}.
    \label{eq:hedge_initiation}
\end{equation}

Contracts for which no eligible initiation exists,
or which lack an exact expiration-date observation,
are excluded. For each retained contract, the
observations from index $i_0-L+1$ through expiration
are preserved.

The moneyness and maturity restrictions are imposed
only at hedge initiation. Subsequent valid observations
are retained even when the contract moves outside the
specified moneyness or maturity intervals. This
path-preserving selection procedure avoids the
truncation of hedging trajectories that would otherwise
result from applying these restrictions independently
to every observation.

\paragraph{Time to maturity.}

Time to maturity is calculated using the Actual/365 Fixed
(ACT/365F) day-count convention. Let $u_t$ denote the
timestamp of observation $t$ and let $u_T^\star$ denote
the prescribed terminal settlement timestamp. For a
live observation, the annualized time to maturity is
given by
\begin{equation}
    \tau_t =
    \frac{
        \operatorname{ElapsedSeconds}(u_t,u_T^\star)
    }{
        365 \times 86400
    },
    \qquad t<T.
    \label{eq:act365_maturity}
\end{equation}

The observation timestamp is assigned to 16:00
New York time for live observations. The nominal
terminal settlement timestamp is assigned to 09:30
for DJX and 16:00 for XEO on the expiration date.
At the terminal observation, $\tau_T=0$ is imposed.

The elapsed time between successive observations,
used subsequently for financing and dividend
accounting, is calculated under the same day-count
convention.

\paragraph{Risk-free rate construction.}

A maturity-dependent risk-free rate is assigned to each
option observation using the U.S. Treasury par yield
curve. To avoid the use of future interest rate
information, each observation is matched to the most
recent available Treasury curve on or before its
observation date, subject to a maximum permissible
difference of seven calendar days.

Let $R_u(d_j)$ denote the Treasury par yield, expressed
as a percentage, at maturity $d_j$ on the matched
Treasury observation date $u$. For an option with
$D_t$ calendar days remaining to expiration, such that
$d_j \leq D_t \leq d_{j+1}$, the corresponding annual
rate is calculated by linear interpolation:
\begin{equation}
\begin{aligned}
    r_t = \frac{1}{100}
    \Bigg[
        R_u(d_j)
        &+
        \frac{D_t-d_j}{d_{j+1}-d_j}
        \Big(
            R_u(d_{j+1})-R_u(d_j)
        \Big)
    \Bigg].
\end{aligned}
\label{eq:treasury_interpolation}
\end{equation}

When the option maturity lies outside the available
Treasury maturity range, the nearest available
endpoint yield is used. Observations for which no
valid Treasury curve is available within the prescribed
time tolerance are not silently imputed.

The resulting Treasury par yield is used as a proxy
for the continuously compounded pricing and financing
rate. It does not represent a bootstrapped zero-coupon
yield curve or a separately estimated short-term
funding curve.

\paragraph{Dividend yield estimation.}

The dividend yield associated with each underlying
index is approximated using the historical prices
and cash distributions of its corresponding ETF
proxy. DIA is used for DJX, while OEF is used for XEO.

Let $P_u^{\mathrm{ETF}}$ denote the unadjusted closing
price of the corresponding ETF on date $u$, and let
$A_v^{\mathrm{ETF}}$ denote its cash distribution
per share on date $v$. The annual dividend yield proxy
is calculated as
\begin{equation}
    q_u =
    \frac{
        \displaystyle
        \sum_{v:\,u-365\mathrm{d}<v\leq u}
        A_v^{\mathrm{ETF}}
    }{
        P_u^{\mathrm{ETF}}
    }.
    \label{eq:dividend_yield_proxy}
\end{equation}

This estimator uses only distributions observed during
the preceding 365 calendar days. A complete one-year
historical warm-up period is required before a dividend
yield is assigned.

For each option observation, the dividend yield is
obtained from the most recent available ETF observation
on or before the corresponding option observation date,
subject to a maximum staleness of seven calendar days.
This backward-only alignment prevents future dividend
distributions from entering the feature representation.

\paragraph{Feature engineering and rolling windows.}

Following the construction of the financial variables,
each option observation is represented by the
six-dimensional feature vector
\begin{equation}
    \mathbf{x}_t =
    \begin{bmatrix}
        \log(S_t/K) &
        \log K &
        \tau_t &
        r_t &
        \nu_t &
        q_t
    \end{bmatrix}^{\top}
    \in \mathbb{R}^{6},
    \label{eq:option_feature_vector}
\end{equation}
where $\nu_t$ denotes the observed implied volatility.

The logarithmic transformations provide a relative
representation of the underlying level with respect
to the strike while retaining information about the
absolute scale of the contract. The remaining variables
describe the maturity, financing conditions, implied
volatility, and estimated dividend yield.

To incorporate the historical evolution of the option
state, a rolling window of length $L=20$ is constructed
for each eligible observation:
\begin{equation}
    \mathbf{X}_t =
    \begin{bmatrix}
        \mathbf{x}_{t-L+1}^{\top} \\
        \mathbf{x}_{t-L+2}^{\top} \\
        \vdots \\
        \mathbf{x}_{t}^{\top}
    \end{bmatrix}
    \in \mathbb{R}^{L\times 6}.
    \label{eq:rolling_option_window}
\end{equation}

The window contains the current observation and the
preceding $L-1$ retained observations of the same
contract. The corresponding price variable is
\begin{equation}
    y_t = V_t^{\mathrm{obs}},
    \label{eq:observed_price_target}
\end{equation}
where $V_t^{\mathrm{obs}}$ denotes the observed option
premium recorded at the final observation of the
window.

Thus, the price variable, underlying level, and
contract features correspond to the same observation
date. The sequence construction does not use future
observations to estimate the current option state.

The resulting windows are assembled into individual
contract paths. Each complete hedging path contains
at least one live observation and a separate exact
expiration observation. Invalid live samples are
excluded, while invalid terminal samples trigger
an explicit error rather than silently truncating
the path. Missing or invalid terminal implied
volatility may be represented by a finite zero
placeholder because the terminal observation is
used for settlement rather than model evaluation.

\paragraph{Chronological data partitioning.}

The complete contract paths are divided into training,
validation, and testing sets using their expiration
dates rather than individual observations. This
ensures that observations belonging to the same
contract are not distributed across multiple
partitions.

Let
\begin{equation}
    \mathcal{E}
    =
    \{e_1,e_2,\ldots,e_m\},
    \qquad
    e_1<e_2<\cdots<e_m,
\end{equation}
denote the ordered set of distinct expiration dates
within an experimental dataset. The training and
validation boundaries are defined by
\begin{equation}
\begin{aligned}
    e_{\mathrm{tr}}
    &= e_{\lfloor 0.6m \rfloor}, \\
    e_{\mathrm{val}}
    &= e_{\lfloor 0.8m \rfloor}.
\end{aligned}
\label{eq:expiration_boundaries}
\end{equation}

For a complete hedging path $p$, let $b(p)$ and $e(p)$
denote its hedge-initiation and expiration dates,
respectively. The training, validation, and testing
partitions are constructed as
\begin{equation}
\begin{aligned}
    \mathcal{D}_{\mathrm{train}}
    &=
    \{p:e(p)\leq e_{\mathrm{tr}}\},\\
    \mathcal{D}_{\mathrm{val}}
    &=
    \{p:b(p)>e_{\mathrm{tr}},
          \ e(p)\leq e_{\mathrm{val}}\},\\
    \mathcal{D}_{\mathrm{test}}
    &=
    \{p:b(p)>e_{\mathrm{val}}\}.
\end{aligned}
\label{eq:purged_chronological_split}
\end{equation}

Validation and testing paths whose hedge initiation
overlaps the preceding partition boundary are removed.
Consequently, the nominal $60:20:20$ partition applies
to distinct expiration dates rather than the final
number of contracts.

The purging procedure ensures that the terminal
outcomes of training paths precede the hedge
initiation of validation paths, and that the terminal
outcomes of validation paths precede the hedge
initiation of testing paths. Historical lookback
observations may precede a partition boundary, but
they contain only information available before the
corresponding hedge-initiation date.

The resulting partitions are held fixed across all
comparative models and random seeds.

\input{tables/dataset_splits}

\paragraph{Data normalization.}

To reduce differences in numerical scale between the
input variables, feature-wise MinMax normalization
is applied. Let $x_j^{\min}$ and $x_j^{\max}$ denote
the minimum and maximum values of the $j$-th feature
across all timesteps of the live training windows,
respectively. For a non-constant feature, the
normalized value is calculated as
\begin{equation}
    \widetilde{x}_{t,j}
    =
    \frac{
        x_{t,j}-x_j^{\min}
    }{
        x_j^{\max}-x_j^{\min}
    },
    \qquad j=1,\ldots,6.
    \label{eq:feature_minmax}
\end{equation}

Similarly, the observed option premium is normalized
using
\begin{equation}
    \widetilde{y}_t
    =
    \frac{
        y_t-y^{\min}
    }{
        y^{\max}-y^{\min}
    },
    \label{eq:target_minmax}
\end{equation}
where $y^{\min}$ and $y^{\max}$ are obtained from
the live training price observations.

The inverse transformation of the normalized model
output is given by
\begin{equation}
    \widehat{V}_t
    =
    (y^{\max}-y^{\min})
    \widehat{y}_t^{\mathrm{norm}}
    +y^{\min}.
    \label{eq:inverse_price_normalization}
\end{equation}

Both feature and price normalization parameters are
estimated exclusively from the live training samples.
The same transformations are subsequently applied to
the validation and testing observations without
refitting or clipping their normalized values.
Consequently, observations outside the training
feature ranges may have normalized values outside
$[0,1]$.

The normalization parameters are retained for
denormalizing the estimated option prices and
rescaling their derivatives to the original
financial units. This preserves consistency between
the normalized model representation and the
subsequent hedging calculations.


==> sections/04_experiments/evaluation_metrics.tex <==

\subsection{Evaluation Metrics}
\label{subsec:evaluation_metrics}

To evaluate the effectiveness of the comparative models
in dynamic option hedging, we consider three performance
metrics: mean squared hedging profit and loss
($\mathrm{PnL}^2$), mean hedging PnL (Mean PnL), and
standard deviation of hedging PnL (Std PnL).
These metrics quantify the magnitude, systematic bias,
and dispersion of terminal replication errors,
respectively.

Let $P_i$ denote the realized terminal hedging PnL
of the $i$-th option contract, obtained through the
self-financing hedging procedure described in
Section~\ref{subsec:hedging_training}, and let $N$
denote the total number of complete option paths
in the test set. The evaluation metrics are defined
as follows.

\paragraph{Mean squared hedging PnL ($\mathrm{PnL}^2$).}

The mean squared hedging PnL measures the magnitude
of terminal replication errors by assigning greater
penalties to large deviations from perfect
replication. It is defined as
\begin{equation}
    \mathrm{PnL}^2
    =
    \frac{1}{N}
    \sum_{i=1}^{N}P_i^2.
    \label{eq:metric_pnl2}
\end{equation}

Lower values indicate better hedging performance.
This metric also serves as the primary optimization
objective for the hedge-trained neural models.

\paragraph{Mean hedging PnL (Mean PnL).}

The mean hedging PnL measures the systematic bias
of the hedging portfolio relative to its terminal
option liability. It is defined as
\begin{equation}
    \mathrm{Mean\ PnL}
    =
    \overline{P}
    =
    \frac{1}{N}
    \sum_{i=1}^{N}P_i.
    \label{eq:metric_mean_pnl}
\end{equation}

Negative and positive values indicate average
replication shortfalls and surpluses, respectively.
Since the objective is accurate replication rather
than profit maximization, values closer to zero
are preferred.

\paragraph{Standard deviation of hedging PnL (Std PnL).}

The standard deviation of hedging PnL measures the
dispersion of terminal replication errors across
option contracts. It is calculated using the
population standard deviation:
\begin{equation}
    \mathrm{Std\ PnL}
    =
    \sqrt{
        \frac{1}{N}
        \sum_{i=1}^{N}
        (P_i-\overline{P})^2
    }.
    \label{eq:metric_std_pnl}
\end{equation}

Lower values indicate more consistent hedging
outcomes across the evaluated contracts.

The three metrics are related through the
bias--variance decomposition
\begin{equation}
    \mathrm{PnL}^2
    =
    (\mathrm{Mean\ PnL})^2
    +
    (\mathrm{Std\ PnL})^2.
    \label{eq:pnl_bias_variance}
\end{equation}

Thus, minimizing squared hedging PnL requires
controlling both systematic replication bias and
the dispersion of hedging errors.

All three metrics assign equal weight to each
complete option path. Mean PnL and Std PnL are
expressed in index points, whereas $\mathrm{PnL}^2$
is expressed in squared index points. For neural
models, the metrics are calculated independently
for each training seed and subsequently averaged
across seeds. The bias--variance identity in
Equation~\eqref{eq:pnl_bias_variance} holds within
each individual evaluation before seed averaging.


==> sections/04_experiments/experimental_setup.tex <==

\subsection{Experimental Setup}
\label{subsec:experimental_setup}

All experiments are conducted independently on the
four option datasets described in
Section~\ref{subsec:data_description}.
The comparative models use identical training,
validation, and testing partitions constructed
according to the procedure described in
Section~\ref{subsec:data_preprocessing}.
The lookback length is fixed at $L=20$, and each
input observation contains $D=6$ financial features.
The experimental setup is designed to maintain
consistent information availability, hedging
conventions, and model selection criteria across
the comparative models.

\paragraph{Common price-interval constraint.}

To maintain financially admissible price levels,
all neural pricing models are equipped with the
same differentiable European option price-interval
transformation. Let
\begin{equation}
    A_t=S_t e^{-q_t\tau_t},
    \qquad
    B_t=K e^{-r_t\tau_t},
\end{equation}
where $q_t$ denotes the dividend yield proxy and
$r_t$ denotes the maturity-dependent risk-free
rate.

The lower and upper price bounds for European
call and put options are defined as
\begin{equation}
    (\underline{V}_t,\overline{V}_t)
    =
    \begin{cases}
        (\max(A_t-B_t,0),A_t),
        & a=C,\\
        (\max(B_t-A_t,0),B_t),
        & a=P,
    \end{cases}
    \label{eq:european_price_bounds}
\end{equation}
where $a\in\{C,P\}$ denotes the option type.

Rather than applying a hard projection to the
unconstrained model output, we employ the smooth
positive-part approximation
\begin{equation}
    g_{\varepsilon}(z)
    =
    \frac{z+\sqrt{z^2+\varepsilon^2}}{2},
    \qquad \varepsilon>0.
    \label{eq:smooth_positive_part}
\end{equation}

Let $v_t$ denote the unconstrained model prediction
after inverse normalization. The bounded option
price is given by
\begin{equation}
\begin{aligned}
    \widehat{V}_t
    = \underline{V}_t
    &+g_{\varepsilon}(v_t-\underline{V}_t)\\
    &-g_{\varepsilon}(v_t-\overline{V}_t).
\end{aligned}
\label{eq:smooth_price_constraint}
\end{equation}

The transformation parameter is fixed at
$\varepsilon=0.1$ index points for all neural
models and experimental datasets. The bounded
price is subsequently mapped back to the
normalized output space.

The transformation is applied during training,
validation, and testing. Consequently, the
model-implied delta is obtained by differentiating
the bounded pricing function, including the
dependence of the interval bounds on the current
underlying level.

This common constraint ensures that differences
in neural hedging performance are not attributable
to the exclusive use of pointwise price bounds
by any individual architecture. The constraint
enforces the specified price interval but does
not impose additional static no-arbitrage
conditions, such as monotonicity, convexity,
or put--call parity.

\paragraph{Hedging and optimization protocol.}

All neural models are optimized using the squared
terminal delta-hedging PnL objective. Unlike
conventional supervised option pricing, the
primary training procedure does not minimize
the discrepancy between predicted and observed
option premiums.

For a mini-batch $\mathcal{B}_j$ containing
complete option paths, the training objective is
\begin{equation}
    \mathcal{L}_j(\theta)
    =
    \frac{1}{|\mathcal{B}_j|}
    \sum_{p\in\mathcal{B}_j}
    P_{\theta}(p)^2,
    \label{eq:experimental_training_loss}
\end{equation}
where $P_{\theta}(p)$ denotes the terminal
hedging PnL obtained using model parameters
$\theta$ along path $p$.

Each mini-batch consists of complete option
paths rather than independent observations.
The ordering of the training paths is randomly
permuted at the beginning of each epoch, while
the chronological ordering of observations
within each path is preserved.

The model-implied delta is calculated through
automatic differentiation with respect to the
current log-moneyness coordinate and rescaled
to the original financial units. The derivative
calculation retains the computational graph
during training, allowing gradients of the
terminal hedging loss to propagate through
the model-implied hedge ratios.

All neural models use the Adam optimizer.
To improve numerical stability, the global
parameter-gradient norm is clipped to a
maximum value of $5$ before each parameter
update. Non-finite training losses and
parameter gradients trigger an explicit
termination of the corresponding training
run.

The baseline hedging portfolio consists of a
short option position, a position in the
underlying, and a cash account. The portfolio
is initialized using the observed option
premium rather than the model-predicted
premium. Interest accrual, dividend income,
rebalancing, and terminal settlement follow
the common self-financing accounting procedure
described in Section~\ref{subsec:hedging_training}.

Between available observations, the previous
underlying position is maintained. The primary
evaluation assumes zero transaction costs and
does not introduce additional option instruments
for gamma or vega hedging. Alternative execution
and market assumptions are examined separately
in the market-realism experiments.

\paragraph{Hyperparameter optimization.}

Hyperparameter optimization is performed
independently for each neural model, experimental
dataset, and random seed using the Tree-structured
Parzen Estimator (TPE) implemented in Hyperopt.

The search procedure jointly considers
model-specific architectural parameters and
optimization parameters, including the learning
rate and the number of complete option paths
per mini-batch.

For each candidate configuration, a maximum
of $40$ training epochs is permitted, with an
early-stopping patience of $3$ epochs.
A total of $25$ hyperparameter trials is
allocated to each search.

Validation is performed after every epoch
using the complete validation partition.
The objective used for hyperparameter
selection is
\begin{equation}
    \mathcal{J}_{\mathrm{val}}(\theta)
    =
    \frac{1}{|\mathcal{D}_{\mathrm{val}}|}
    \sum_{p\in\mathcal{D}_{\mathrm{val}}}
    P_{\theta}(p)^2.
    \label{eq:hyperparameter_selection}
\end{equation}

Let $\boldsymbol{\lambda}$ denote a candidate
hyperparameter configuration and let
$\theta_{\boldsymbol{\lambda}}^{\star}$ denote
its validation-selected model parameters.
The selected hyperparameter configuration is
\begin{equation}
    \boldsymbol{\lambda}^{\star}
    =
    \underset{
        \boldsymbol{\lambda}
        \in\mathcal{H}_{25}
    }{\arg\min}
    \;
    \mathcal{J}_{\mathrm{val}}
    \left(
        \theta_{\boldsymbol{\lambda}}^{\star}
    \right),
    \label{eq:optimal_hyperparameters}
\end{equation}
where $\mathcal{H}_{25}$ denotes the set of
configurations evaluated during the corresponding
hyperparameter search.

The model-specific search spaces are summarized
in Table~\ref{tab:neural-hyperparameter-space}.
Learning rates are sampled on a logarithmic
scale, dropout probabilities are sampled
uniformly over their specified intervals, and
discrete architectural parameters are selected
from predefined candidate sets.

\input{tables/hyperparameter_search}

The common trial budget, epoch limits, and
validation objective standardize the search
protocol across neural architectures.
However, the computational cost of an
individual trial may differ according to
model complexity, mini-batch size, and
the number of epochs completed before
early stopping.

\paragraph{Final training and model selection.}

Following hyperparameter optimization,
the selected architectural configuration,
learning rate, and path-batch size are
retained for final training. A new model
is initialized and trained exclusively
on the training partition for a maximum
of $200$ epochs, with an early-stopping
patience of $5$ epochs.

The validation partition is not merged
with the training partition. Validation
hedging loss is evaluated after every
epoch and used to determine the model
checkpoint retained for testing.

Let $\theta_e$ denote the model parameters
after training epoch $e$. The selected
checkpoint is given by
\begin{equation}
    e^{\star}
    =
    \underset{
        1\leq e\leq E_{\mathrm{stop}}
    }{\arg\min}
    \;
    \mathcal{J}_{\mathrm{val}}(\theta_e),
    \qquad
    \theta^{\star}=\theta_{e^{\star}},
    \label{eq:final_checkpoint_selection}
\end{equation}
where $E_{\mathrm{stop}}\leq 200$ denotes
the number of epochs completed before
training terminates.

The selected parameters are restored
before evaluating the model on the
held-out test partition. The testing
partition is not used for hyperparameter
optimization, early stopping, or checkpoint
selection.

Algorithms~\ref{alg:pathwise_evaluation}
and~\ref{alg:hedge_loss_training} summarize
the pathwise evaluation and neural model
training procedures, respectively.

\input{algorithms/pathwise_evaluation}
\input{algorithms/hedge_loss_training}

\paragraph{Configuration of classical models.}

The classical and numerical pricing models
use the observed market implied volatility
at each live observation. The current
underlying level, strike price, time to
maturity, risk-free rate, and dividend
yield proxy are obtained using the same
financial data and accounting conventions
as those employed by the neural models.

For the Merton jump-diffusion model, the
jump intensity, mean logarithmic jump
size, and jump-size standard deviation
are held fixed. For the Heston model,
the initial instantaneous variance at
each valuation time is set to
\begin{equation}
    v_{0,t}=\nu_t^2,
    \label{eq:heston_initial_variance}
\end{equation}
while the remaining stochastic volatility
parameters are held fixed.

The binomial and finite difference models
use fixed numerical discretizations.
The complete configurations are reported
in Table~\ref{tab:classical_configurations}.

\input{tables/classical_configurations}

No additional parameter calibration or
hyperparameter optimization is performed
for the classical and numerical models.
Consequently, these comparisons evaluate
the specified market-IV-driven baseline
configurations rather than exhaustively
calibrated stochastic pricing models.

\paragraph{Reproducibility and implementation.}

The neural experiments are repeated using
five random seeds,
\begin{equation}
    \mathcal{S}=\{40,41,42,43,44\}.
\end{equation}

For each seed, hyperparameter optimization
and final model training are performed
independently. Random number generators
in Python, NumPy, and PyTorch are initialized
using the corresponding seed.

The same contract partitions are retained
across all seeds and comparative models.
Therefore, variation across neural runs
reflects stochastic training and
hyperparameter selection rather than
variation in the test contract population.

The final hedging metrics are calculated
independently for each run and averaged
across the five seeds, following the
evaluation conventions described in
Section~\ref{subsec:evaluation_metrics}.
Each deterministic classical model is
evaluated once per experimental dataset.

The neural experiments are implemented
using PyTorch 2.4.1 and NumPy 1.26.4,
with hyperparameter optimization performed
using Hyperopt. The saved protocol
manifests identify CPU-based PyTorch
execution for the primary neural
comparison.

The source code, experimental
configurations, and associated evaluation
procedures are retained to support
reproducibility of the reported results.


==> sections/05_results/ablation_study.tex <==
\begin{table}[!htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.05}
\caption{HARP-Net architectural ablation: selected configurations.}
\label{tab:ablation-djx-module-table}
\begin{adjustbox}{max width=\linewidth}
\begin{threeparttable}
\begin{tabular}{@{}lcccccccrr@{}}
\toprule
\textbf{Case}
& \textbf{P} & \textbf{R} & \textbf{T} & \textbf{D}
& \textbf{F} & \textbf{B} & \textbf{G}
& \multicolumn{2}{c}{\textbf{Normalized average}} \\
\cmidrule(lr){9-10}
& & & & & & & & \textbf{PnL$^2$} & \textbf{Std} \\
\midrule
I
& \checkmark & \checkmark & \checkmark & \checkmark
& \checkmark & \checkmark & \checkmark
& \textbf{1.0000} & \textbf{1.0000} \\
II
& \checkmark & $\times$ & $\times$ & $\times$
& $\times$ & $\times$ & $\times$
& 1.1016 & 1.0535 \\
III
& \checkmark & \checkmark & $\times$ & $\times$
& \checkmark & $\times$ & $\times$
& 1.0160 & 1.0062 \\
IV
& \checkmark & \checkmark & $\times$ & \checkmark
& \checkmark & \checkmark & \checkmark
& 1.0078 & 1.0041 \\
V
& \checkmark & $\times$ & \checkmark & \checkmark
& \checkmark & \checkmark & \checkmark
& 1.1028 & 1.0522 \\
VI
& \checkmark & \checkmark & \checkmark & $\times$
& \checkmark & \checkmark & \checkmark
& 1.0734 & 1.0333 \\
VII
& \checkmark & \checkmark & \checkmark & \checkmark
& $\times$ & \checkmark & \checkmark
& 1.0102 & 1.0052 \\
IX
& \checkmark & \checkmark & \checkmark & \checkmark
& \checkmark & \checkmark & $\times$
& 1.1003 & 1.0414 \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\scriptsize\raggedright
\item \textit{Note.} Checkmarks denote active components.
Metrics are arithmetic means of task-level ratios to the fresh
full-model control across DJX/XEO calls and puts; lower is better.
Each task metric is first averaged over seeds 40--44, except the
deterministic Black--Scholes reference. Bold marks the minimum
among the displayed configurations.

P: Black--Scholes prior;
R: residual anchor;
T: temporal encoder;
D: domain embeddings;
F: current-feature skip;
B: bridge refinement;
G: velocity gate.
I: full model;
II: Black--Scholes only;
III: BS + current-state MLP;
IV--VII and IX: individual component removals.
The gate is inactive when the bridge is disabled.
One validation-selected full-model configuration per task is held
fixed across learned variants and seeds.
The full model equals 1 by construction.
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
\end{table}

==> sections/05_results/computational_efficiency_robustness.tex <==

\subsection{Computational Efficiency and Robustness}
\label{subsec:computational_efficiency}

Table~\ref{tab:computational-efficacy} presents the
computational efficiency of the comparative models.
HARP-Net contains approximately $107.1$K parameters,
requires an average training time of $5.9$ minutes
per seed, and evaluates a complete hedging path in
$13.21$ ms. Despite its moderate parameter count,
HARP-Net achieves the lowest aggregate hedging error
among the comparative models. Its reported evaluation
time is lower than those of Heston and FDM, although
hardware equivalence between the classical and neural
experiments has not been established. These results
indicate a favorable trade-off between hedging
performance and computational efficiency.

\input{tables/computational_efficacy}

Table~\ref{tab:robustness-seed-pnl2} presents the
robustness of the comparative neural models across
five independent training seeds. HARP-Net achieves
the lowest mean PnL$^2$ and the lowest standard
deviation across seeds among the selected neural
baselines on all four datasets. These results
indicate consistent hedging performance across
independent training runs.

\input{tables/robustness}


==> sections/05_results/distributional_tail_risk/distribution_of_absolute_hedging_error.tex <==
\subsubsection{Distribution of Absolute Hedging Error}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/absolute-pnl-ecdf-full.pdf}
    \caption{Empirical cumulative distribution functions (ECDFs) of absolute test-path hedging errors.}
    \label{fig:absolute-pnl-ecdf-grid}
\end{figure}

Figure~\ref{fig:absolute-pnl-ecdf-grid} complements the aggregate metrics by showing the complete distribution of absolute pathwise error. HARP-Net generally produces faster-rising curves, particularly on DJX Call, XEO Call, and XEO Put, indicating smaller errors for a larger fraction of paths. The curves are more closely grouped on the VIX tasks, consistent with the smaller differences observed in Table~\ref{tab:hedging_summary}. Thus, the overall improvements are distributional rather than being driven only by a few extreme observations.

==> sections/05_results/distributional_tail_risk/tail_risk_comparison.tex <==
\subsubsection{Tail-Risk Comparison}
\label{subsec:tail-risk-comparison}

Figures~\ref{fig:tail-risk-cvar95-abs-pnl-grid}--%
\ref{fig:appendix-tail-risk-q99-abs-pnl-grid} examine large absolute
terminal hedging errors through three complementary measures:
$\mathrm{CVaR}_{95}(|\mathrm{PnL}|)$,
$Q_{95}(|\mathrm{PnL}|)$, and
$Q_{99}(|\mathrm{PnL}|)$.
Lower values indicate smaller extreme replication errors.
Because the metrics use absolute PnL, they capture both positive
and negative deviations from perfect replication, rather than
the downside losses of a signed trading portfolio.

Each metric is computed separately within each training seed
and then averaged across seeds $40$--$44$.
Black-Scholes and Merton contribute one deterministic evaluation
per task. Quantiles use linear interpolation, while
$\mathrm{CVaR}_{95}$ is calculated as the mean absolute PnL
at or above the empirical 95th-percentile threshold.
In finite samples, threshold ties can make the included tail
larger than exactly $5\%$ of paths.

HARP-Net achieves the lowest seed-mean
$\mathrm{CVaR}_{95}(|\mathrm{PnL}|)$ among the six compared models
on all four DJX/XEO call/put tasks.
Its values are $7.1542$, $8.2497$, $86.6824$, and $99.9302$
for DJX Call, DJX Put, XEO Call, and XEO Put, respectively.
Relative to Black-Scholes, these correspond to reductions of
$7.57\%$, $1.21\%$, $10.18\%$, and $1.37\%$.
The strongest improvements therefore occur on the call tasks,
while the put-task advantages over the classical reference
are comparatively small.


\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.96\linewidth]
    {figures/tail-risk-cvar95.pdf}
    \caption{
    Tail-risk comparison using
    $\mathrm{CVaR}_{95}(|\mathrm{PnL}|)$ on held-out
    DJX and XEO call/put paths.
    Within each run, the metric is the mean absolute terminal
    hedging error at or above its empirical 95th percentile;
    threshold ties are included.
    Neural metrics are averaged across seeds $40$--$44$,
    while classical references are deterministic.
    Values are in index points; lower is better.
    }
    \label{fig:tail-risk-cvar95-abs-pnl-grid}
\end{figure}

The percentile comparisons show a similar but less uniform
pattern. HARP-Net has the lowest $Q_{95}$ and $Q_{99}$ on
DJX Call, DJX Put, and XEO Call.
On XEO Put, GRU achieves the lowest $Q_{95}$ at $85.6003$,
compared with $86.0475$ for HARP-Net.
Black-Scholes achieves the lowest $Q_{99}$ on that task
at $106.3343$, compared with $107.4748$ for HARP-Net.
Thus, the favorable CVaR results do not imply dominance
at every tail threshold.


\begin{figure}[!htbp]
\centering
    \includegraphics[width=0.84\linewidth]
    {figures/tail-risk-q95.pdf}
    \caption{
    Empirical 95th percentile of absolute terminal
    hedging PnL, $Q_{95}(|\mathrm{PnL}|)$,
    on held-out DJX and XEO call/put paths.
    Quantiles are computed within each run using linear
    interpolation and then averaged across seeds $40$--$44$
    for neural models.
    Classical references are deterministic.
    Values are in index points; lower is better.
    }
    \label{fig:appendix-tail-risk-q95-abs-pnl-grid}
\par\smallskip
\centering
    \includegraphics[width=0.84\linewidth]
    {figures/tail-risk-q99.pdf}
    \caption{
    Empirical 99th percentile of absolute terminal
    hedging PnL, $Q_{99}(|\mathrm{PnL}|)$,
    on held-out DJX and XEO call/put paths.
    Quantiles are computed within each run using linear
    interpolation and then averaged across seeds $40$--$44$
    for neural models.
    Classical references are deterministic.
    Values are in index points; lower is better.
    }
    \label{fig:appendix-tail-risk-q99-abs-pnl-grid}
\end{figure}

Across the four tasks, the equally weighted mean ratios
to the corresponding Black-Scholes metric are $0.9229$
for $Q_{95}$, $0.9537$ for $Q_{99}$, and $0.9492$ for
$\mathrm{CVaR}_{95}$.
These dimensionless summaries indicate average relative
reductions of $7.71\%$, $4.63\%$, and $5.08\%$, respectively,
without pooling raw errors across underlyings with different
index-point scales.

Overall, the results support improved control of large absolute
replication errors under the evaluated protocol, with exceptions
at individual percentile thresholds.
They do not establish statistical significance or superiority
in unseen market periods.
In particular, the DJX panels contain only $99$ call and $100$
put contracts, with five contracts contributing to each
within-run CVaR estimate, so their extreme-tail estimates
have limited sample resolution.


==> sections/05_results/greek_quality_diagnostics.tex <==
\subsection{Greek Quality Diagnostics}
\label{subsec:greek-quality}

Figures~\ref{fig:greek-quality-pooled-overview}--
\ref{fig:greek-quality-vega-diagnostic-grid}
examine complementary aspects of the derivative behavior of
the saved hedge-trained pricing models without direct Greek
supervision. Eight diagnostics are evaluated on matched held-out
DJX and XEO call/put observations: delta smoothness, delta turnover,
mean absolute gamma, mean absolute vega, delta correlation with
Black-Scholes, Greek explosion rate, and gamma- and vega-attribution
residual MSEs. Neural results are computed separately for each
seed and averaged across seeds $40$--$44$; Black-Scholes and
Merton are deterministic references. Model deltas are obtained
through automatic differentiation, while gamma and vega are
estimated using finite differences. Historical window inputs
remain fixed when perturbing current-state features.

\paragraph{Delta regularity.}
Figure~\ref{fig:greek-quality-pooled-overview} reports delta
smoothness and turnover. For a path with live hedge positions
$\Delta_0,\ldots,\Delta_{T-1}$, these quantities are defined as
\[
\mathrm{Smoothness}
=
\frac{1}{T-1}
\sum_{t=1}^{T-1}|\Delta_t-\Delta_{t-1}|,
\qquad
\mathrm{Turnover}
=
|\Delta_0|
+
\sum_{t=1}^{T-1}|\Delta_t-\Delta_{t-1}|.
\]
A path containing only one live observation has zero smoothness
and turnover equal to $|\Delta_0|$. Both diagnostics are averaged
across paths within each run before averaging across seeds.
Turnover measures initial entry and subsequent hedge adjustments;
it excludes terminal liquidation.

HARP-Net's seed-mean smoothness ranges from $0.0583$ to $0.0751$
across the four tasks, compared with $0.0584$ to $0.0775$ for
Black-Scholes. Its turnover is lower than Black-Scholes on
both call tasks and slightly higher on both put tasks.
These results indicate hedge-position variation close to the
analytical reference. However, low smoothness or turnover can
also arise from an under-responsive hedge and must therefore
be interpreted alongside terminal hedging performance.

\paragraph{Derivative magnitudes and reference agreement.}
Figure~\ref{fig:greek-quality-magnitudes} reports mean absolute
gamma and vega across live observations. Gamma is expressed
in price points per squared spot point, while vega is expressed
in price points per one volatility percentage point.
HARP-Net's mean absolute gamma ranges from $0.00249$ to
$0.01753$, and its mean absolute vega per volatility point
ranges from $0.2624$ to $1.8396$ across the four tasks.
These magnitudes describe the responsiveness of the pricing
surface; smaller values are not automatically more accurate.

The Pearson correlation between HARP-Net's model-implied
delta and the Black--Scholes delta, averaged across seeds,
ranges from $0.9964$ to approximately $1.0000$ across the
four datasets, indicating close agreement with the
analytical reference. However, such agreement does not
establish ground-truth Greek accuracy or imply that
the reference hedge is optimal under all market conditions.

\paragraph{Numerical stability}
The explosion-rate diagnostic flags nonfinite derivatives
or observations satisfying $|\Delta|>2$, $|\Gamma|>10$,
or $|\nu_{\mathrm{point}}|>100$.
No nonfinite evaluations or threshold exceedances are observed
across the $88$ model/task/seed evaluations.
Since all models satisfy these thresholds, the diagnostic
does not distinguish their relative numerical stability.

Additional half- and double-bump checks flag numerical
sensitivity in $1$ of $20$ HARP-Net runs, compared with
$20$ of $20$ PAttn runs and $17$ of $20$ runs for both GRU
and NLinear. A run is flagged when the sampled
95th-percentile relative change exceeds $25\%$ for either Greek.
These checks support comparatively stable HARP-Net finite-difference
estimates under the tested perturbations, although relative
changes can be inflated when the underlying derivative is
close to zero.

\paragraph{Gamma and vega attribution residuals.}
Figures~\ref{fig:greek-quality-gamma-diagnostic-grid} and
\ref{fig:greek-quality-vega-diagnostic-grid} report squared
Taylor-attribution residuals constructed from common-capital
delta-hedging PnL. For a path $p$, the gamma diagnostic is
\[
R_\Gamma(p)
=
P_\Delta(p)
-
\frac{1}{2}
\sum_{t=0}^{T-1}
\Gamma_t(S_{t+1}-S_t)^2.
\]
The terminal increment uses the prescribed underlying
settlement mark, including DJS settlement for DJX.
The vega diagnostic is
\[
R_\nu(p)
=
P_\Delta(p)
-
\sum_{t=0}^{T-2}
\nu_t^{\mathrm{raw}}(\sigma_{t+1}-\sigma_t),
\]
where $\nu_t^{\mathrm{raw}}$ denotes vega per unit change in
decimal volatility. Only consecutive live implied-volatility
observations enter this correction; terminal placeholder
volatility is excluded. Each reported diagnostic is the
mean squared pathwise residual, subsequently averaged
across seeds for neural models.

HARP-Net has the lowest gamma residual MSE among the six
compared models on DJX Call, DJX Put, and XEO Call;
GRU has the lowest value on XEO Put.
For the vega residual, HARP-Net is lowest on the two DJX
tasks, while GRU is lowest on the two XEO tasks.
These task-dependent rankings show that lower terminal
hedging PnL$^2$ does not imply the lowest value of every
derivative diagnostic.

The attribution residuals omit theta, carry, and higher-order
terms. They are not self-financing portfolios that trade
additional options, and their rankings should not be interpreted
as evidence of executable gamma- or vega-hedging superiority.
Taken together, the diagnostics support finite, reference-aligned,
and comparatively bump-insensitive HARP-Net derivatives on
the evaluated test observations. They do not establish
ground-truth Greek accuracy, global arbitrage freedom,
statistical significance, or universal superiority.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.49\textwidth]
    {figures/delta-smoothness.pdf}
    \hfill
    \includegraphics[width=0.49\textwidth]
    {figures/delta-turnover.pdf}
    \caption{
    Delta smoothness (left) and delta turnover (right) on
    matched held-out DJX and XEO call/put paths.
    Smoothness is the mean absolute consecutive delta change
    within each path; turnover includes the absolute initial
    position and subsequent absolute position changes,
    excluding terminal liquidation.
    Path-level quantities are averaged within each run,
    then across seeds $40$--$44$ for neural models.
    Classical references are deterministic.
    Smaller values indicate less hedge-position variation
    and should be interpreted alongside hedging performance.
    }
    \label{fig:greek-quality-pooled-overview}
\end{figure}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.49\textwidth]
    {figures/gamma-magnitude.pdf}
    \hfill
    \includegraphics[width=0.49\textwidth]
    {figures/vega-magnitude.pdf}
    \caption{
    Mean absolute gamma (left) and vega (right) on matched
    live test observations.
    Gamma is expressed in price points per squared spot point;
    vega is expressed in price points per one volatility
    percentage point.
    Observation-level magnitudes are averaged within each run,
    then across seeds $40$--$44$ for neural models.
    Classical references are deterministic.
    Derivative magnitude measures sensitivity and is not
    independently a lower-is-better accuracy criterion.
    }
    \label{fig:greek-quality-magnitudes}
\end{figure}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.95\textwidth]
    {figures/gamma-diag-pnl-mse.pdf}
    \caption{
    Mean squared gamma-attribution residual on held-out option
    paths. The residual subtracts the accumulated
    $\tfrac12\Gamma_t(\Delta S_t)^2$ contribution from
    common-capital delta-hedging PnL.
    Neural metrics are averaged across seeds $40$--$44$.
    Values are squared index points.
    This incomplete Taylor residual is a diagnostic,
    not the PnL of an executable gamma-hedging portfolio.
    }
    \label{fig:greek-quality-gamma-diagnostic-grid}
\end{figure}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.95\textwidth]
    {figures/vega-diag-pnl-mse.pdf}
    \caption{
    Mean squared vega-attribution residual on held-out option
    paths. The residual subtracts raw-unit vega multiplied
    by consecutive live implied-volatility changes from
    common-capital delta-hedging PnL.
    Terminal placeholder volatility is excluded.
    Neural metrics are averaged across seeds $40$--$44$.
    Values are squared index points.
    This diagnostic does not represent an executable
    vega-hedging portfolio.
    }
    \label{fig:greek-quality-vega-diagnostic-grid}
\end{figure}

==> sections/05_results/main_hedging_results.tex <==



==> sections/05_results/market_realism.tex <==
\subsection{Market-Realism Analysis}
\label{subsec:market-realism}

Figures~\ref{fig:market-realism-execution}--%
\ref{fig:market-realism-liquidity} examine whether the trained hedging
models retain their performance under alternative execution and
portfolio-management assumptions. The study replays saved models
without retraining on the same held-out DJX and XEO call/put paths.
Neural results are arithmetic averages of per-seed metrics across
seeds 40--44; Black-Scholes and Merton are deterministic references.
The comparisons cover initial option proceeds, proportional
underlying transaction costs, rebalancing frequency, symmetric
position limits, and an initiation-time liquidity filter.

Figure~\ref{fig:market-realism-execution} compares initialization
using the observed option premium, the arithmetic bid--ask mid,
the option bid, and the model-implied price.
The observed-premium case is the clean evaluation control.
Bid execution represents the proceeds received from selling the
option, whereas model-price initialization supplies different
initial capital to different models and is therefore a
counterfactual rather than a common-capital execution comparison.
HARP-Net has the lowest seed-mean PnL$^2$ among the six compared
models on all four tasks under observed-premium, market-mid,
and option-bid initialization.

Figures~\ref{fig:market-realism-transaction-costs} and
\ref{fig:market-realism-transaction-cost-mean} introduce proportional
underlying trading costs of $0$, $1$, $5$, and $10$ basis points,
with initial option proceeds fixed at the bid.
Costs apply to initial hedge entry, subsequent rebalancing,
and terminal liquidation. HARP-Net retains the lowest mean
PnL$^2$ in all $16$ task/cost-level comparisons.
At $10$ basis points, its PnL$^2$ is $13.2291$, $14.9590$,
$2239.9740$, and $2395.7197$ for DJX Call, DJX Put,
XEO Call, and XEO Put, respectively, compared with
$14.6986$, $15.1703$, $2476.9734$, and $2508.6947$
for Black-Scholes.
The corresponding mean-PnL figure documents the effect of
trading-cost deductions on signed replication errors.
These comparisons describe sensitivity under the specified
cost assumptions and do not constitute independent statistical
tests across cost levels.


\begin{figure}[!htbp]
\centering
    \includegraphics[width=0.84\linewidth]
    {figures/execution-pnl2.pdf}
    \caption{
    Test hedging PnL$^2$ under alternative initial option proceeds:
    observed premium, model-implied price, arithmetic market mid,
    and option bid.
    Model-price initialization is a counterfactual with
    model-dependent initial capital.
    Neural metrics are averaged across seeds 40--44;
    classical references are deterministic.
    Lower values indicate smaller squared replication errors.
    }
    \label{fig:market-realism-execution}
\par\smallskip
\centering
    \includegraphics[width=0.84\linewidth]
    {figures/transaction-cost-pnl2.pdf}
    \caption{
    Test hedging PnL$^2$ under option-bid initialization and
    proportional underlying transaction costs of
    $0$, $1$, $5$, and $10$ basis points.
    Costs include initial hedge entry, rebalancing,
    and terminal liquidation.
    Neural metrics are averaged across seeds 40--44.
    }
    \label{fig:market-realism-transaction-costs}
\end{figure}

Figure~\ref{fig:market-realism-rebalancing} evaluates hedge updates
scheduled every one, two, or five observed market dates.
Between updates, the existing underlying position is held while
cash financing and dividend-proxy income continue to accrue.
If a scheduled contract quote is unavailable, execution waits
until the next available quote.
HARP-Net has the lowest mean PnL$^2$ on all four tasks at each
tested frequency, although the absolute effect of less frequent
rebalancing varies across tasks.
For example, moving from daily to five-date rebalancing increases
HARP-Net's PnL$^2$ from $8.0579$ to $21.9114$ on DJX Call,
whereas XEO Put changes from $1070.6976$ to $1038.2227$.
Thus, reduced trading frequency does not uniformly increase
squared replication error in the observed sample.


\begin{figure}[!htbp]
\centering
    \includegraphics[width=0.84\linewidth]
    {figures/transaction-cost-mean-pnl.pdf}
    \caption{
    Signed mean terminal hedging PnL under option-bid
    initialization and proportional underlying trading costs.
    Neural metrics are averaged across seeds 40--44.
    Mean PnL measures replication bias; closeness to zero,
    rather than a more negative value, is desirable.
    }
    \label{fig:market-realism-transaction-cost-mean}
\par\smallskip
\centering
    \includegraphics[width=0.84\linewidth]
    {figures/rebalance-frequency-pnl2.pdf}
    \caption{
    Test hedging PnL$^2$ when hedge updates are scheduled every
    one, two, or five observed market dates.
    Positions are held between updates, with financing and
    dividend-proxy income accrued over elapsed time.
    Missing scheduled contract quotes defer execution to the
    next available observation.
    These scenarios use observed initial option proceeds
    and zero transaction costs.
    }
    \label{fig:market-realism-rebalancing}
\end{figure}

Figure~\ref{fig:market-realism-position-limits} imposes symmetric
hedge-position bounds, $|h_t|\leq c$, for
$c\in\{1,2,5,10\}$, alongside an unlimited-position control.
Symmetric clipping preserves negative put hedge positions.
The limits of $2$, $5$, and $10$ are nonbinding in these runs;
their unchanged results should therefore be interpreted as
controls. A limit of $1$ affects some paths, but HARP-Net
retains the lowest mean PnL$^2$ across the four tasks.
Frequency and position-limit experiments use observed initial
option proceeds and zero transaction costs, so they measure
separate scenario effects rather than a combined execution stress.

Figure~\ref{fig:market-realism-liquidity} evaluates a common subset
of contracts satisfying initial volume $\geq1$, open interest
$\geq1$, and relative bid--ask spread $\leq0.5$.
The filter retains $31$ DJX calls and $47$ DJX puts.
HARP-Net's PnL$^2$ is $4.4497$ and $11.2741$ on these subsets,
compared with $5.0447$ and $11.4774$ for Black-Scholes.
No XEO test contracts satisfy all filters, so XEO liquid-subset
results are unavailable. Differences between the full sample
and the liquidity subset reflect a change in the evaluated
contract population and should not be interpreted as a causal
effect of liquidity.


\begin{figure}[!htbp]
\centering
    \includegraphics[width=0.84\linewidth]
    {figures/position-limit-pnl2.pdf}
    \caption{
    Test hedging PnL$^2$ under symmetric underlying-position
    limits of $1$, $2$, $5$, and $10$, compared with
    unrestricted positions.
    Limits of $2$ or greater are nonbinding in the evaluated runs.
    Scenarios use observed initial option proceeds,
    daily scheduled updates, and zero transaction costs.
    }
    \label{fig:market-realism-position-limits}
\par\smallskip
\centering
    \includegraphics[width=0.84\linewidth]
    {figures/liquidity-subset-pnl2.pdf}
    \caption{
    Test hedging PnL$^2$ on a common initiation-time liquidity
    subset requiring volume $\geq1$, open interest $\geq1$,
    and relative bid--ask spread $\leq0.5$.
    The subset contains $31$ DJX calls and $47$ DJX puts.
    No XEO contracts pass all filters; their results are
    unavailable rather than zero.
    Neural metrics are averaged across seeds 40--44.
    }
    \label{fig:market-realism-liquidity}
\end{figure}

All scenarios require complete paths with terminal $\tau_T=0$,
consistent with the saved expiry dates and settlement conventions.
DJX option payoff and synthetic underlying liquidation use the
verified DJS settlement value; terminal observations are not
rebalancing dates.
The study therefore avoids evaluating silently truncated
pre-expiry paths.
Its results remain conditional on synthetic index/basket
hedging, Treasury financing and dividend proxies, and the
specified execution-cost assumptions. They establish descriptive
robustness under these scenarios rather than fully executable
trading performance or universal superiority.


==> sections/05_results/statistical_significance/mcs_test.tex <==
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{0.96}
\begin{longtable}{@{}llrrrrrr@{}}
\caption{Model Confidence Set (MCS) p-values
    with respect to squared hedging PnL,
    absolute mean PnL, and standard deviation
    of PnL on the test set.
    Bold values indicate membership in the
    Model Confidence Set at the 5\% significance level.}
    \label{tab:mcs_test} \\
\toprule
\textbf{Model} & \textbf{Index} & \multicolumn{2}{c}{\textbf{PnL$^2$}} & \multicolumn{2}{c}{\textbf{$|\mathrm{Mean\ PnL}|$}} & \multicolumn{2}{c}{\textbf{Std PnL}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & \textbf{C} & \textbf{P} & \textbf{C} & \textbf{P} & \textbf{C} & \textbf{P} \\
\midrule\endfirsthead
\toprule
\textbf{Model} & \textbf{Index} & \multicolumn{2}{c}{\textbf{PnL$^2$}} & \multicolumn{2}{c}{\textbf{$|\mathrm{Mean\ PnL}|$}} & \multicolumn{2}{c}{\textbf{Std PnL}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & \textbf{C} & \textbf{P} & \textbf{C} & \textbf{P} & \textbf{C} & \textbf{P} \\
\midrule\endhead
\bottomrule\endfoot
Black-Scholes & DJX & \best{0.080} & \best{0.071} & $<0.001$ & 0.002 & 0.046 & 0.007 \\*
 & XEO & \best{0.120} & \best{0.139} & $<0.001$ & 0.005 & \best{1.000} & \best{0.182} \\
Heston & DJX & \best{0.073} & 0.041 & $<0.001$ & $<0.001$ & $<0.001$ & $<0.001$ \\*
 & XEO & 0.021 & \best{0.120} & $<0.001$ & $<0.001$ & $<0.001$ & 0.017 \\
Merton & DJX & 0.005 & 0.009 & $<0.001$ & $<0.001$ & $<0.001$ & $<0.001$ \\*
 & XEO & $<0.001$ & \best{0.126} & $<0.001$ & $<0.001$ & \best{0.372} & \best{0.182} \\
Binomial & DJX & \best{0.080} & \best{0.071} & $<0.001$ & 0.044 & 0.046 & $<0.001$ \\*
 & XEO & \best{0.120} & \best{0.139} & $<0.001$ & 0.004 & \best{0.643} & \best{0.182} \\
FDM & DJX & 0.001 & 0.011 & \best{0.207} & \best{1.000} & $<0.001$ & $<0.001$ \\*
 & XEO & \best{0.087} & \best{0.139} & $<0.001$ & $<0.001$ & 0.006 & $<0.001$ \\
MLP & DJX & $<0.001$ & 0.019 & \best{0.207} & $<0.001$ & $<0.001$ & $<0.001$ \\*
 & XEO & 0.047 & 0.003 & 0.007 & $<0.001$ & $<0.001$ & $<0.001$ \\
DLinear & DJX & \best{0.080} & \best{0.071} & \best{0.146} & 0.003 & $<0.001$ & $<0.001$ \\*
 & XEO & \best{0.070} & \best{0.126} & 0.014 & $<0.001$ & $<0.001$ & $<0.001$ \\
NLinear & DJX & \best{0.080} & 0.027 & 0.030 & 0.003 & $<0.001$ & $<0.001$ \\*
 & XEO & 0.047 & \best{0.073} & $<0.001$ & \best{0.526} & $<0.001$ & $<0.001$ \\
ResNet & DJX & 0.005 & \best{0.071} & \best{0.207} & \best{0.357} & $<0.001$ & $<0.001$ \\*
 & XEO & $<0.001$ & 0.015 & $<0.001$ & \best{0.504} & $<0.001$ & $<0.001$ \\
LSTM & DJX & 0.005 & \best{0.057} & \best{0.051} & 0.012 & $<0.001$ & $<0.001$ \\*
 & XEO & \best{0.070} & 0.003 & 0.014 & \best{0.124} & $<0.001$ & $<0.001$ \\
GRU & DJX & \best{0.080} & \best{0.071} & $<0.001$ & 0.037 & $<0.001$ & $<0.001$ \\*
 & XEO & \best{0.070} & 0.033 & 0.014 & \best{0.340} & $<0.001$ & $<0.001$ \\
CNN-1D & DJX & 0.018 & \best{0.071} & \best{0.207} & $<0.001$ & $<0.001$ & $<0.001$ \\*
 & XEO & $<0.001$ & 0.003 & $<0.001$ & 0.016 & $<0.001$ & $<0.001$ \\
CNN-LSTM & DJX & \best{0.080} & \best{0.071} & \best{0.063} & 0.002 & $<0.001$ & $<0.001$ \\*
 & XEO & 0.023 & \best{0.079} & $<0.001$ & \best{1.000} & $<0.001$ & $<0.001$ \\
CNN-BiLSTM & DJX & \best{0.060} & \best{0.071} & \best{0.207} & $<0.001$ & $<0.001$ & $<0.001$ \\*
 & XEO & 0.047 & 0.042 & $<0.001$ & \best{0.634} & $<0.001$ & $<0.001$ \\
Transformer & DJX & 0.018 & $<0.001$ & 0.006 & $<0.001$ & $<0.001$ & $<0.001$ \\*
 & XEO & 0.021 & $<0.001$ & 0.007 & \best{0.783} & $<0.001$ & $<0.001$ \\
DeepAR & DJX & \best{0.056} & $<0.001$ & 0.006 & 0.020 & $<0.001$ & $<0.001$ \\*
 & XEO & \best{0.068} & 0.015 & 0.001 & \best{0.129} & $<0.001$ & $<0.001$ \\
PAttn & DJX & \best{0.080} & \best{0.071} & \best{0.189} & \best{0.212} & $<0.001$ & $<0.001$ \\*
 & XEO & \best{0.070} & \best{0.139} & 0.001 & 0.048 & $<0.001$ & 0.003 \\
TimeXer & DJX & 0.018 & \best{0.071} & 0.028 & \best{0.271} & $<0.001$ & $<0.001$ \\*
 & XEO & $<0.001$ & \best{0.139} & \best{0.432} & \best{0.284} & $<0.001$ & $<0.001$ \\
WPMixer & DJX & \best{0.056} & 0.037 & 0.028 & \best{0.357} & $<0.001$ & $<0.001$ \\*
 & XEO & 0.047 & \best{0.126} & $<0.001$ & \best{0.330} & $<0.001$ & $<0.001$ \\
HARP-Net & DJX & \best{1.000} & \best{1.000} & \best{1.000} & \best{0.470} & \best{1.000} & \best{1.000} \\*
 & XEO & \best{1.000} & \best{1.000} & \best{1.000} & \best{0.783} & \best{0.643} & \best{1.000} \\
\end{longtable}

\endgroup


==> sections/05_results/statistical_significance/statistical_significance.tex <==

\subsection{Statistical Significance}
\label{subsec:statistical-comparison}

To assess whether the observed differences in hedging
performance are statistically supported, we employ
Diebold--Mariano (DM) equal-loss tests and the Model
Confidence Set (MCS) procedure.

For each dataset, the terminal hedging errors are
grouped chronologically by expiration date. Let
$\mathcal{G}_g$ denote the set of option contracts
associated with expiration group $g$, and let
$N_g=|\mathcal{G}_g|$. The group-level losses are
defined as
\begin{align}
    L_{g,1}
    &=
    \frac{1}{N_g}
    \sum_{i\in\mathcal{G}_g}P_i^2,
    \\
    L_{g,2}
    &=
    \left|\overline{P}_g\right|,
    \\
    L_{g,3}
    &=
    \sqrt{
        \frac{1}{N_g}
        \sum_{i\in\mathcal{G}_g}
        (P_i-\overline{P}_g)^2
    },
    \label{eq:statistical_group_losses}
\end{align}
where $\overline{P}_g$ denotes the mean terminal
PnL within expiration group $g$.

Groups containing fewer than two contracts are
excluded. For neural models, the group-level losses
are calculated independently for each training seed
and subsequently averaged across seeds. This avoids
treating repeated evaluations of identical market
observations as independent samples. Unlike the
metrics in Section~\ref{subsec:evaluation_metrics},
the statistical comparisons assign equal weight
to expiration groups rather than individual contracts.

\subsubsection{Diebold--Mariano Test}

For each benchmark model $m$, the loss differential
relative to HARP-Net is defined as
\begin{equation}
    d_g=L_{m,g}-L_{\mathrm{HARP},g},
\end{equation}
where a positive value favors HARP-Net.

The null hypothesis of equal expected loss is
$H_0:\mathbb{E}[d_g]=0$. The test statistic is
computed as
\begin{equation}
    \mathrm{DM}
    =
    \frac{\overline{d}}
    {\sqrt{\widehat{\Omega}/G}},
    \label{eq:dm_statistic}
\end{equation}
where $G$ denotes the number of eligible expiration
groups and $\widehat{\Omega}$ is the Newey--West
heteroskedasticity- and autocorrelation-consistent
estimate of the long-run variance of the loss
differential.

Bartlett weights are employed with truncation lag
\begin{equation}
    \ell
    =
    \min\left\{
        \left\lfloor
            4(G/100)^{2/9}
        \right\rfloor,
        G-2
    \right\}.
\end{equation}

Two-sided asymptotic p-values are calculated using
the standard normal distribution. Holm's procedure
is applied jointly across all dataset, metric,
and benchmark comparisons to control the
family-wise error rate at the 5\% significance level.

As summarized in Table~\ref{tab:statistical_summary},
the adjusted tests identify significantly lower
PnL$^2$ for HARP-Net in six of the 76 pairwise
comparisons, all associated with the XEO datasets.
Stronger evidence is obtained for Std PnL, for
which 62 of the 76 comparisons favor HARP-Net
after multiplicity correction. For absolute Mean
PnL, the corresponding number is 27.

No adjusted rejection favors a comparative model.
However, failure to reject equal expected loss
does not establish equivalence between models.

\subsubsection{Model Confidence Set}

The MCS procedure identifies a subset of models
that cannot be statistically distinguished under
the specified loss criterion and confidence level.
For an active model set $\mathcal{M}$, the range
statistic is defined as
\begin{equation}
    T_R
    =
    \max_{i,j\in\mathcal{M},\,i\neq j}
    \left|
        \frac{\overline{d}_{ij}}
        {\widehat{\mathrm{se}}
        (\overline{d}_{ij})}
    \right|,
    \label{eq:mcs_range_statistic}
\end{equation}
where $\overline{d}_{ij}$ denotes the mean
loss differential between models $i$ and $j$.

The sampling distribution is estimated using
9,999 stationary bootstrap replications, with
expected block length
$\max(2,\lfloor\sqrt{G}\rfloor)$.
Models are sequentially eliminated according
to their maximum standardized adverse loss
differential to construct the 95\% confidence set.

HARP-Net is retained in the confidence set for
all twelve dataset--metric combinations.
For Std PnL, it is the sole retained model on
both DJX datasets, while it remains alongside
Black--Scholes, Merton, and Binomial on both
XEO datasets. The confidence sets for PnL$^2$
contain several competing models, indicating
that the observed improvements in squared
hedging error cannot be statistically
distinguished from all benchmarks.

\input{tables/statistical_summary}

Overall, the statistical comparisons provide
stronger evidence for reductions in hedging
error dispersion than for reductions in squared
hedging error or absolute replication bias.
Nevertheless, the limited number of expiration
groups, particularly for DJX, and the dependence
induced by overlapping hedging intervals
restrict the strength of statistical inference.
The results should therefore be interpreted
conditional on the observed market sample and
trained model configurations, rather than as
evidence of universal statistical superiority.


==> subsections/algorithm.tex <==

\subsection{Algorithm}
\label{app:algo}
% ============================================================

For completeness, Algorithms~\ref{alg:pathwise_evaluation} and~\ref{alg:hedge_loss_training} summarize
the evaluation and training procedures used for the proposed hedging-aware pricing
framework. The model operates on normalized rolling option-state
sequences and is optimized through the mean squared terminal
delta-hedging PnL. At each rebalancing time, the model-implied delta
is obtained by automatic differentiation with respect to the
current log-moneyness input and rescaled to the original price
and underlying scales. Historical inputs in the rolling window
are held fixed when computing this derivative.

The hedging portfolio represents a short option position financed
by the observed initial option premium. Its cash balance accrues
at the previous observation's Treasury rate, and dividend-proxy
income is credited on the previous underlying position.
Rebalancing trades are funded from the cash account.
The final holding interval includes the same financing and
dividend accounting before the portfolio is liquidated against
the terminal option payoff. Gradients are propagated through
the model-implied deltas and the resulting pathwise hedging PnL.

Here, $\Delta t_t$ denotes the elapsed ACT/365F time between observations $t-1$ and $t$, using the prescribed observation clocks. The terminal underlying mark $S_T^\star$ corresponds to DJS settlement for DJX and the expiry underlying close for XEO. The initial capital $V_0^{\mathrm{obs}}$ is the raw observed option premium.

% ============================================================
% Algorithm 1: Pathwise hedging evaluation
% ============================================================

\begin{algorithm}[!htbp]
\caption{Pathwise Delta-Hedging PnL Evaluation}
\label{alg:pathwise_evaluation}
\small

\setlength{\abovedisplayskip}{4pt}
\setlength{\belowdisplayskip}{4pt}

\begin{algorithmic}[1]

\Require Complete option path $p$, pricing model $f_\theta$,
option style $a\in\{C,P\}$, train-fitted scalers.

\Ensure Terminal hedging PnL $P_\theta(p)$.

\State Let $\ell_t=\log(S_t/K)$ and let $s_y$, $s_\ell$
denote the inverse MinMax scaling coefficients.

\State Compute the model-implied delta at each live observation:
\[
\widehat{\Delta}_t
=
\frac{s_y}{s_\ell S_t}
\frac{
\partial f_\theta(\widetilde{x}_{t,\mathrm{seq}})
}{
\partial\widetilde{\ell}_t
}.
\]

\State Define the terminal payoff:
\[
\Phi_a(S_T^\star,K)=
\begin{cases}
\max(S_T^\star-K,0), & a=C,\\
\max(K-S_T^\star,0), & a=P.
\end{cases}
\]

\State Initialize the underlying holding and cash account:
\[
h_0=\widehat{\Delta}_0,
\qquad
c_0=V_0^{\mathrm{obs}}-h_0S_0.
\]

\For{$t=1,\ldots,T-1$}

    \State Accrue interest and dividend income:
    \[
    c_t^- =
    c_{t-1}e^{r_{t-1}\Delta t_t}
    +h_{t-1}S_{t-1}q_{t-1}\Delta t_t.
    \]

    \State Rebalance the underlying position:
    \[
    \begin{aligned}
    c_t &= c_t^-
    -(\widehat{\Delta}_t-h_{t-1})S_t,\\
    h_t &= \widehat{\Delta}_t.
    \end{aligned}
    \]

\EndFor

\State Accrue the final holding interval:
\[
c_T^- =
c_{T-1}e^{r_{T-1}\Delta t_T}
+h_{T-1}S_{T-1}q_{T-1}\Delta t_T.
\]

\State Compute terminal hedging PnL:
\[
P_\theta(p)=
c_T^-+h_{T-1}S_T^\star-\Phi_a(S_T^\star,K).
\]

\State \Return $P_\theta(p)$.

\end{algorithmic}
\end{algorithm}


% ============================================================
% Algorithm 2: Model optimization
% ============================================================

\begin{algorithm}[!htbp]
\caption{Pathwise Delta Hedge-Loss Training}
\label{alg:hedge_loss_training}
\small

\setlength{\abovedisplayskip}{4pt}
\setlength{\belowdisplayskip}{4pt}

\begin{algorithmic}[1]

\Require Training paths $\mathcal{D}_{\mathrm{train}}$,
validation paths $\mathcal{D}_{\mathrm{val}}$,
pricing model $f_\theta$, learning rate $\eta$,
path-batch size $B$, maximum epochs $E$,
early-stopping patience $p_{\mathrm{stop}}$.

\Ensure Validation-selected parameters $\theta^\star$.

\State Initialize Adam with learning rate $\eta$.
\State Initialize the best validation loss to $+\infty$.

\For{$e=1,\ldots,E$}

    \State Set the model to training mode.

    \State Partition $\mathcal{D}_{\mathrm{train}}$
    into path mini-batches $\{\mathcal{B}_j\}$.

    \For{each mini-batch $\mathcal{B}_j$}

        \State Clear accumulated parameter gradients.

        \For{each path $p\in\mathcal{B}_j$}

            \State Evaluate $P_\theta(p)$ using
            Algorithm~\ref{alg:pathwise_evaluation},
            retaining the autograd graph.

        \EndFor

        \State Compute the batch loss:
        \[
        \mathcal{L}_j=
        \frac{1}{|\mathcal{B}_j|}
        \sum_{p\in\mathcal{B}_j}P_\theta(p)^2.
        \]

        \State Backpropagate $\mathcal{L}_j$.
        \State Clip the parameter-gradient norm to $5$.
        \State Update $\theta$ using Adam.

    \EndFor

    \State Set the model to evaluation mode.

    \State Evaluate validation paths using autograd
    without retaining higher-order training graphs.

    \State Compute the validation loss:
    \[
    \mathcal{L}_{\mathrm{val}}=
    \frac{1}{|\mathcal{D}_{\mathrm{val}}|}
    \sum_{p\in\mathcal{D}_{\mathrm{val}}}P_\theta(p)^2.
    \]

    \State Save $\theta$ as $\theta^\star$
    if validation loss improves.

    \State Stop if validation loss does not improve
    for $p_{\mathrm{stop}}$ consecutive epochs.

\EndFor

\State Restore and \Return $\theta^\star$.

\end{algorithmic}
\end{algorithm}

The training loss assigns equal weight to each complete option
path in a mini-batch. Interest accrues on the signed cash balance,
and dividend income is approximated using the previous holding,
underlying level, dividend yield, and elapsed time.
The baseline training objective includes no transaction costs
or additional gamma/vega hedging instruments.
Terminal evaluation requires $\tau_T=0$; the terminal observation
is used for settlement rather than rebalancing.
Model selection uses the complete validation set after every epoch,
and the checkpoint with the lowest validation hedging PnL$^2$
is restored before test evaluation.
The maximum epoch count and patience are $(40,3)$ during tuning
and $(200,5)$ during final training.

==> subsections/hyperparameter_tuning.tex <==
\subsection{Hyperparameter Tuning and Implementation Details}

Hyperparameter search spaces for the hedge-trained neural models are
summarized in Table~\ref{tab:neural-hyperparameter-space}.
Hyperparameter optimization is performed separately for each model,
dataset/style task, and random seed using Hyperopt's Tree-structured
Parzen Estimator (TPE), with $25$ trials per search.
Each trial is trained for at most $40$ epochs, with early-stopping
patience of $3$. Validation is performed after every epoch using the
complete validation set. Both hyperparameter selection and early
stopping use validation delta-hedging PnL$^2$.

The selected architecture, learning rate, and path-batch size are
retained for final training. A freshly initialized model is then
trained on the training partition for at most $200$ epochs, with
early-stopping patience of $5$. The validation partition remains
separate and is used for checkpoint selection; it is not merged into
the training data. The checkpoint with the lowest validation
hedging loss is restored before test evaluation.



\begingroup
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.10}
\begin{longtable}{@{}>{\raggedright\arraybackslash}p{0.18\linewidth}>{\raggedright\arraybackslash}p{0.47\linewidth}>{\raggedright\arraybackslash}p{0.28\linewidth}@{}}
\caption{
Hyperparameter search spaces for hedge-trained neural models.
Learning rates are sampled log-uniformly, and dropout rates uniformly
over the stated intervals. Discrete sets specify candidate values.
Each search uses $25$ TPE trials, with at most $40$ epochs per trial
and early-stopping patience of $3$.
Batch paths denotes the number of complete option paths per
optimization batch.
}\label{tab:neural-hyperparameter-space} \\

\toprule
\textbf{Model} & \textbf{Architecture hyperparameters}
& \textbf{Optimization hyperparameters} \\
\midrule
\endfirsthead

\toprule
\textbf{Model} & \textbf{Architecture hyperparameters}
& \textbf{Optimization hyperparameters} \\
\midrule
\endhead
\bottomrule
\endfoot

MLP
& hidden dimension $\in \{8,16,32,64\}$;
layers $\in \{1,2,3,4\}$
& learning rate $\in [10^{-4},10^{-2}]$;
batch paths $\in \{8,12,16,24\}$ \\
\addlinespace[3pt]
LSTM
& hidden size $\in \{32,64,96\}$;
layers $\in \{1,2\}$; dropout $\in [0,0.3]$
& learning rate $\in [10^{-4},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16,24\}$ \\
\addlinespace[3pt]
GRU
& hidden size $\in \{32,64,96,128\}$;
layers $\in \{1,2,3\}$; dropout $\in [0,0.4]$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16,24\}$ \\
\addlinespace[3pt]
Transformer
& model width $\in \{32,64,96\}$;
heads $\in \{2,4,8\}$;
encoder layers $\in \{1,2,3\}$;
feed-forward width $\in \{128,192,256\}$;
dropout $\in [0,0.2]$
& learning rate $\in [10^{-4},10^{-2}]$;
batch paths $\in \{4,6,8,12\}$ \\
\addlinespace[3pt]
ResNet
& base channels $\in \{16,32,64\}$;
residual blocks $\in \{2,3,4\}$;
kernel size $\in \{3,5\}$
& learning rate $\in [10^{-4},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16\}$ \\
\addlinespace[3pt]
DLinear
& moving-average kernel $\in \{3,4,5,8,10,12,16,25\}$;
individual channel head $\in \{\mathrm{false},\mathrm{true}\}$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16,24\}$ \\
\addlinespace[3pt]
NLinear
& individual channel head $\in \{\mathrm{false},\mathrm{true}\}$;
channel dependence $\in \{2,4,8,16\}$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16,24\}$ \\
\addlinespace[3pt]
DeepAR
& recurrent hidden size $\in \{32,64,96,128\}$;
recurrent layers $\in \{1,2,3\}$;
dropout $\in [0,0.4]$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16,24\}$ \\
\addlinespace[3pt]
CNN1D
& channels $\in \{32,64,96\}$;
depth $\in \{2,3,4\}$;
kernel size $\in \{3,5\}$;
dropout $\in [0,0.3]$
& learning rate $\in [10^{-4},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16\}$ \\
\addlinespace[3pt]
CNN-LSTM
& convolution channels $\in \{16,32,64\}$;
LSTM hidden size $\in \{32,64,96\}$;
LSTM layers $\in \{1,2\}$;
dropout $\in [0,0.3]$
& learning rate $\in [10^{-4},10^{-2}]$;
batch paths $\in \{6,8,12,16\}$ \\
\addlinespace[3pt]
CNN-BiLSTM
& convolution channels $\in \{16,32,64\}$;
kernel size $\in \{3,5\}$;
LSTM hidden size $\in \{32,64,96\}$;
LSTM layers $\in \{1,2\}$;
dropout $\in [0,0.3]$
& learning rate $\in [10^{-4},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16\}$ \\
\addlinespace[3pt]
DDMLP
& domain channels $\in \{3,4,5,6\}$;
domain hidden dimension $\in \{32,64,96,128\}$;
domain layers $\in \{1,2,3,4\}$;
domain embedding dimension $\in \{8,16,32\}$;
head hidden dimension $\in \{16,32,64\}$;
dropout $\in [0,0.3]$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16,24\}$ \\
\addlinespace[3pt]
PAttn
& model width $\in \{32,64,96\}$;
feed-forward width $\in \{64,128,192\}$;
heads $\in \{2,4,8\}$;
patch length $\in \{4,8,10\}$;
stride $\in \{2,4\}$;
dropout $\in [0,0.2]$;
head hidden dimension $\in \{16,32,64\}$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{4,6,8,12\}$ \\
\addlinespace[3pt]
TimeXer
& model width $\in \{32,64,96\}$;
feed-forward width $\in \{64,128,192\}$;
heads $\in \{2,4,8\}$;
encoder layers $\in \{1,2\}$;
patch length $\in \{2,4,5,10\}$;
dropout $\in [0,0.2]$;
head hidden dimension $\in \{16,32,64\}$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{4,6,8,12\}$ \\
\addlinespace[3pt]
WPMixer
& model width $\in \{32,64,96\}$;
feed-forward width $\in \{64,128,192\}$;
heads $\in \{2,4,8\}$;
patch length $\in \{2,4,5,10\}$;
stride $\in \{2,4\}$;
temporal factor $\in \{3,5\}$;
feature factor $\in \{3,5\}$;
wavelet level $=1$;
dropout $\in [0,0.2]$;
head hidden dimension $\in \{16,32,64\}$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{4,6,8,12\}$ \\
\addlinespace[3pt]
HARP-Net
& domains $=3$;
latent dimension $\in \{32,64,96\}$;
temporal encoder $=\mathrm{GRU}$;
bridge steps $\in \{2,4\}$;
context layers $\in \{1,2,3\}$;
field layers $\in \{1,2,3\}$;
activation $\in \{\mathrm{GELU},\mathrm{ReLU},\mathrm{SiLU}\}$;
dropout $\in [0,0.15]$;
residual scale $\in \{0.05,0.10,0.25,0.50\}$;
prior correction scale $\in \{0.25,0.50,1.00\}$;
drift clip $\in \{0.02,0.05,0.10\}$
& learning rate $\in [5{\times}10^{-5},2{\times}10^{-3}]$;
batch paths $\in \{8,12,16,24\}$ \\

\end{longtable}
\noindent\scriptsize\raggedright\textit{Note.}
Parameters not listed as search variables retain their configured values.
For HARP-Net, the Black-Scholes prior, residual anchor, bridge refinement,
and gated velocity are enabled; score drift is disabled.
Architecture-removal experiments are conducted separately from this search.
\par
\endgroup



All hedge-trained neural methods use Adam optimization, a maximum
gradient norm of $5$, and mean squared terminal delta-hedging PnL as
the training objective. The lookback length is fixed at $L=20$.
Each input window contains six variables:
log-moneyness $\log(S/K)$, log-strike $\log K$,
time to maturity $\tau$, the maturity-matched Treasury rate $r$,
implied volatility $\sigma$, and dividend yield $q$.
Feature and target MinMax scalers are fitted using live training
observations only and are subsequently applied to validation and test
data without refitting.

Experiments cover DJX and XEO calls and puts.
Complete contract paths are partitioned chronologically by expiration
date, with nominal training/validation/test proportions of
$60\%/20\%/20\%$ of distinct expiration dates.
Paths whose hedge initiation crosses the preceding partition boundary
are purged, and terminal evaluation requires an exact-expiry
observation.
The same path partitions and accounting conventions are used across
the compared methods.

Experiments are repeated with random seeds
$40$, $41$, $42$, $43$, and $44$.
Because tuning is repeated for each seed, variation across seeds
reflects both hyperparameter selection and stochastic training.
Reported neural performance is the arithmetic average of the
per-seed test metrics. Seed-robustness tables additionally report
the sample standard deviation across the five runs.
The common trial count, epoch limits, and validation objective
standardize the search protocol, although actual computational
cost varies with model architecture and early stopping.
The source code and saved experiment configurations will be
made available in the accompanying repository.

==> tables/classical_configurations.tex <==

\begin{table}[!htbp]
    \centering
    \caption{Parameter configurations of the classical
    and numerical option pricing models.}
    \label{tab:classical_configurations}

    \small
    \renewcommand{\arraystretch}{1.15}
    \setlength{\tabcolsep}{5pt}

    \begin{threeparttable}

    \begin{tabular}{
        @{}
        l
        p{0.45\linewidth}
        l
        @{}
    }
        \toprule
        \textbf{Model}
        & \textbf{Parameter}
        & \textbf{Value} \\
        \midrule

        Black--Scholes
        & Volatility $\sigma_t$
        & Market IV \\

        \addlinespace[4pt]

        Merton
        & Jump intensity $\lambda_J$
        & $0.20$ \\
        & Mean log-jump size $\mu_J$
        & $-0.10$ \\
        & Jump standard deviation $\sigma_J$
        & $0.20$ \\
        & Poisson truncation parameter
        & $40$ \\

        \addlinespace[4pt]

        Heston
        & Initial variance $v_{0,t}$
        & $\nu_t^2$ \\
        & Mean-reversion speed $\kappa$
        & $1.50$ \\
        & Long-run variance $\theta_v$
        & $0.04$ \\
        & Volatility of variance $\sigma_v$
        & $0.30$ \\
        & Correlation $\rho$
        & $-0.70$ \\
        & Integration panels
        & $1500$ \\
        & Integration upper limit
        & $100$ \\

        \addlinespace[4pt]

        Binomial
        & Number of tree steps
        & $500$ \\

        \addlinespace[4pt]

        FDM
        & Spatial discretization steps
        & $300$ \\
        & Temporal discretization steps
        & $300$ \\

        \bottomrule
    \end{tabular}

    \begin{tablenotes}[flushleft]
        \footnotesize
        \raggedright
        \item \textit{Note.}
        All models use contemporaneous market implied
        volatility. The structural parameters of
        the Merton and Heston models and the numerical
        discretizations are fixed across datasets.
        No additional parameter calibration is performed.
    \end{tablenotes}

    \end{threeparttable}
\end{table}


==> tables/computational_efficacy.tex <==
\begin{table}[!htbp]
\centering
\caption{Computational efficiency comparison across DJX
and XEO call and put tasks.}
\label{tab:computational-efficacy}

\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.05}

\begin{threeparttable}
\begin{tabular}{@{}lrrrr@{}}
\toprule
\textbf{Model}
& \textbf{Parameters}
& \shortstack{\textbf{Train time}\\(min/seed)}
& \shortstack{\textbf{Test time}\\(ms/path)}
& \shortstack{\textbf{PnL$^2$}\\\textbf{ratio}} \\
\midrule

\multicolumn{5}{@{}l}{\textit{Classical models}} \\
\addlinespace[2pt]

Black-Scholes & -- & --   & 1.30    & 1.14 \\
Merton        & -- & --   & 2.60    & 1.18 \\
Heston        & -- & --   & 47.56   & 1.35 \\
FDM           & -- & --   & 5122.51 & 1.19 \\

\midrule
\multicolumn{5}{@{}l}{\textit{Neural models}} \\
\addlinespace[2pt]

GRU         & 89.1K  & 10.8 & 16.19 & 2.94 \\
NLinear     & 163    & 1.7  & 3.79  & 4.51 \\
PAttn       & 41.9K  & 12.1 & 16.37 & 4.59 \\
LSTM        & 48.4K  & 10.4 & 16.12 & 2.97 \\
TimeXer     & 94.6K  & 17.5 & 23.30 & 4.01 \\
CNN-LSTM    & 68.4K  & 9.4  & 18.78 & 2.48 \\
Transformer & 50.8K  & 3.6  & 6.49  & 2.84 \\
WPMixer     & 87.9K  & 6.1  & 10.34 & 4.22 \\
CNN-BiLSTM  & 185.1K & 19.7 & 34.84 & 2.44 \\
MLP         & 4.3K   & 1.8  & 3.57  & 5.88 \\
DLinear     & 206    & 3.2  & 4.12  & 5.79 \\
DeepAR      & 90.7K  & 11.4 & 22.32 & 3.00 \\
ResNet      & 21.8K  & 5.2  & 9.94  & 3.64 \\
CNN1D       & 23.8K  & 4.0  & 6.92  & 5.67 \\

\midrule
\textbf{HARP-Net}
& 107.1K
& 5.9
& 13.21
& \textbf{1.00} \\

\bottomrule
\end{tabular}

\begin{tablenotes}[flushleft]
\footnotesize
\raggedright

\item \textit{Note.} Parameter counts, final training
times (excluding tuning), and test runtimes per
complete delta-hedging path are averaged over seeds
40--44 and then equally across tasks. Classical methods
use one deterministic evaluation per task. The
PnL$^2$ ratio is the geometric mean of task-level
ratios relative to HARP-Net, using seed-average losses.
CPU timings originate from separate neural and classical
experiments; hardware equivalence is not established.
K denotes thousands of parameters.

\end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/dataset_splits.tex <==

\begin{table}[!htbp]
    \centering
    \caption{Number of complete option paths retained
    in each chronological partition.}
    \label{tab:dataset_splits}

    \small
    \setlength{\tabcolsep}{7pt}
    \renewcommand{\arraystretch}{1.12}

    \begin{threeparttable}
        \begin{tabular}{@{}lrrrr@{}}
            \toprule
            \textbf{Dataset}
            & \textbf{Train}
            & \textbf{Validation}
            & \textbf{Test}
            & \textbf{Total} \\
            \midrule
            DJX-Call & 303   & 87  & 99  & 489   \\
            DJX-Put  & 320   & 90  & 100 & 510   \\
            XEO-Call & 2,180 & 682 & 608 & 3,470 \\
            XEO-Put  & 2,497 & 815 & 786 & 4,098 \\
            \midrule
            \textbf{Total}
            & \textbf{5,300}
            & \textbf{1,674}
            & \textbf{1,593}
            & \textbf{8,567} \\
            \bottomrule
        \end{tabular}

        \begin{tablenotes}[flushleft]
            \footnotesize
            \raggedright
            \item \textit{Note.} Counts are reported
            after final path eligibility checks and
            chronological boundary purging. The nominal
            $60:20:20$ split is applied to distinct
            expiration dates rather than contract counts.
        \end{tablenotes}
    \end{threeparttable}
\end{table}


==> tables/evaluations_metrics.tex <==

\subsection{Evaluation Metrics}
\label{subsec:evaluation_metrics}

To evaluate the effectiveness of the comparative models
in dynamic option hedging, we consider three performance
metrics: mean squared hedging profit and loss
($\mathrm{PnL}^2$), mean hedging PnL (Mean PnL), and
standard deviation of hedging PnL (Std PnL).
These metrics quantify the magnitude, systematic bias,
and dispersion of terminal replication errors,
respectively.

Let $P_i$ denote the realized terminal hedging PnL
of the $i$-th option contract, obtained through the
self-financing hedging procedure described in
Section~\ref{subsec:hedging_training}, and let $N$
denote the total number of complete option paths
in the test set. The evaluation metrics are defined
as follows.

\paragraph{Mean squared hedging PnL ($\mathrm{PnL}^2$).}

The mean squared hedging PnL measures the magnitude
of terminal replication errors by assigning greater
penalties to large deviations from perfect
replication. It is defined as
\begin{equation}
    \mathrm{PnL}^2
    =
    \frac{1}{N}
    \sum_{i=1}^{N}P_i^2.
    \label{eq:metric_pnl2}
\end{equation}

Lower values indicate better hedging performance.
This metric also serves as the primary optimization
objective for the hedge-trained neural models.

\paragraph{Mean hedging PnL (Mean PnL).}

The mean hedging PnL measures the systematic bias
of the hedging portfolio relative to its terminal
option liability. It is defined as
\begin{equation}
    \mathrm{Mean\ PnL}
    =
    \overline{P}
    =
    \frac{1}{N}
    \sum_{i=1}^{N}P_i.
    \label{eq:metric_mean_pnl}
\end{equation}

Negative and positive values indicate average
replication shortfalls and surpluses, respectively.
Since the objective is accurate replication rather
than profit maximization, values closer to zero
are preferred.

\paragraph{Standard deviation of hedging PnL (Std PnL).}

The standard deviation of hedging PnL measures the
dispersion of terminal replication errors across
option contracts. It is calculated using the
population standard deviation:
\begin{equation}
    \mathrm{Std\ PnL}
    =
    \sqrt{
        \frac{1}{N}
        \sum_{i=1}^{N}
        (P_i-\overline{P})^2
    }.
    \label{eq:metric_std_pnl}
\end{equation}

Lower values indicate more consistent hedging
outcomes across the evaluated contracts.

The three metrics are related through the
bias--variance decomposition
\begin{equation}
    \mathrm{PnL}^2
    =
    (\mathrm{Mean\ PnL})^2
    +
    (\mathrm{Std\ PnL})^2.
    \label{eq:pnl_bias_variance}
\end{equation}

Thus, minimizing squared hedging PnL requires
controlling both systematic replication bias and
the dispersion of hedging errors.

All three metrics assign equal weight to each
complete option path. Mean PnL and Std PnL are
expressed in index points, whereas $\mathrm{PnL}^2$
is expressed in squared index points. For neural
models, the metrics are calculated independently
for each training seed and subsequently averaged
across seeds. The bias--variance identity in
Equation~\eqref{eq:pnl_bias_variance} holds within
each individual evaluation before seed averaging.


==> tables/experimental_setup.tex <==
\begin{table}[!htbp]
    \centering
    \caption{Specifications of the option datasets.}
    \label{tab:dataset_spec}

    \small
    \setlength{\tabcolsep}{6pt}
    \renewcommand{\arraystretch}{1.15}

    \begin{threeparttable}
        \begin{tabular}{@{}lrrrrr@{}}
            \toprule
            \textbf{Dataset}
            & \textbf{Observations}
            & \textbf{Contracts}
            & \textbf{ATM}
            & \textbf{ITM}
            & \textbf{OTM} \\
            \midrule
            DJX-Call & 22,038  & 500   & 253   & 122   & 125 \\
            DJX-Put  & 23,284  & 521   & 254   & 142   & 125 \\
            XEO-Call & 122,349 & 3,596 & 1,855 & 1,021 & 720 \\
            XEO-Put  & 138,981 & 4,224 & 1,842 & 1,511 & 871 \\
            \bottomrule
        \end{tabular}

        \begin{tablenotes}[flushleft]
        \footnotesize
        \raggedright
        
        \item \textit{Note.} Contracts denotes the number
        of distinct option contracts. Contracts are classified
        at their first recorded observation: ATM denotes
        $0.96 \leq S/K \leq 1.04$, with ITM and OTM defined
        outside this band according to option type.
        
        \end{tablenotes}
    \end{threeparttable}
\end{table}

==> tables/hyperparameter_search.tex <==
\begingroup
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.10}
\begin{longtable}{@{}>{\raggedright\arraybackslash}p{0.18\linewidth}>{\raggedright\arraybackslash}p{0.47\linewidth}>{\raggedright\arraybackslash}p{0.28\linewidth}@{}}
\caption{
Hyperparameter search spaces for the neural
option pricing models.
}
\label{tab:neural-hyperparameter-space} \\

\toprule
\textbf{Model} & \textbf{Architecture hyperparameters}
& \textbf{Optimization hyperparameters} \\
\midrule
\endfirsthead

\toprule
\textbf{Model} & \textbf{Architecture hyperparameters}
& \textbf{Optimization hyperparameters} \\
\midrule
\endhead
\bottomrule
\endfoot

MLP
& hidden dimension $\in \{8,16,32,64\}$;
layers $\in \{1,2,3,4\}$
& learning rate $\in [10^{-4},10^{-2}]$;
batch paths $\in \{8,12,16,24\}$ \\
\addlinespace[3pt]
LSTM
& hidden size $\in \{32,64,96\}$;
layers $\in \{1,2\}$; dropout $\in [0,0.3]$
& learning rate $\in [10^{-4},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16,24\}$ \\
\addlinespace[3pt]
GRU
& hidden size $\in \{32,64,96,128\}$;
layers $\in \{1,2,3\}$; dropout $\in [0,0.4]$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16,24\}$ \\
\addlinespace[3pt]
Transformer
& model width $\in \{32,64,96\}$;
heads $\in \{2,4,8\}$;
encoder layers $\in \{1,2,3\}$;
feed-forward width $\in \{128,192,256\}$;
dropout $\in [0,0.2]$
& learning rate $\in [10^{-4},10^{-2}]$;
batch paths $\in \{4,6,8,12\}$ \\
\addlinespace[3pt]
ResNet
& base channels $\in \{16,32,64\}$;
residual blocks $\in \{2,3,4\}$;
kernel size $\in \{3,5\}$
& learning rate $\in [10^{-4},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16\}$ \\
\addlinespace[3pt]
DLinear
& moving-average kernel $\in \{3,4,5,8,10,12,16,25\}$;
individual channel head $\in \{\mathrm{false},\mathrm{true}\}$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16,24\}$ \\
\addlinespace[3pt]
NLinear
& individual channel head $\in \{\mathrm{false},\mathrm{true}\}$;
channel dependence $\in \{2,4,8,16\}$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16,24\}$ \\
\addlinespace[3pt]
DeepAR
& recurrent hidden size $\in \{32,64,96,128\}$;
recurrent layers $\in \{1,2,3\}$;
dropout $\in [0,0.4]$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16,24\}$ \\
\addlinespace[3pt]
CNN1D
& channels $\in \{32,64,96\}$;
depth $\in \{2,3,4\}$;
kernel size $\in \{3,5\}$;
dropout $\in [0,0.3]$
& learning rate $\in [10^{-4},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16\}$ \\
\addlinespace[3pt]
CNN-LSTM
& convolution channels $\in \{16,32,64\}$;
LSTM hidden size $\in \{32,64,96\}$;
LSTM layers $\in \{1,2\}$;
dropout $\in [0,0.3]$
& learning rate $\in [10^{-4},10^{-2}]$;
batch paths $\in \{6,8,12,16\}$ \\
\addlinespace[3pt]
CNN-BiLSTM
& convolution channels $\in \{16,32,64\}$;
kernel size $\in \{3,5\}$;
LSTM hidden size $\in \{32,64,96\}$;
LSTM layers $\in \{1,2\}$;
dropout $\in [0,0.3]$
& learning rate $\in [10^{-4},3{\times}10^{-3}]$;
batch paths $\in \{8,12,16\}$ \\
\addlinespace[3pt]
PAttn
& model width $\in \{32,64,96\}$;
feed-forward width $\in \{64,128,192\}$;
heads $\in \{2,4,8\}$;
patch length $\in \{4,8,10\}$;
stride $\in \{2,4\}$;
dropout $\in [0,0.2]$;
head hidden dimension $\in \{16,32,64\}$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{4,6,8,12\}$ \\
\addlinespace[3pt]
TimeXer
& model width $\in \{32,64,96\}$;
feed-forward width $\in \{64,128,192\}$;
heads $\in \{2,4,8\}$;
encoder layers $\in \{1,2\}$;
patch length $\in \{2,4,5,10\}$;
dropout $\in [0,0.2]$;
head hidden dimension $\in \{16,32,64\}$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{4,6,8,12\}$ \\
\addlinespace[3pt]
WPMixer
& model width $\in \{32,64,96\}$;
feed-forward width $\in \{64,128,192\}$;
heads $\in \{2,4,8\}$;
patch length $\in \{2,4,5,10\}$;
stride $\in \{2,4\}$;
temporal factor $\in \{3,5\}$;
feature factor $\in \{3,5\}$;
wavelet level $=1$;
dropout $\in [0,0.2]$;
head hidden dimension $\in \{16,32,64\}$
& learning rate $\in [5{\times}10^{-5},3{\times}10^{-3}]$;
batch paths $\in \{4,6,8,12\}$ \\
\addlinespace[3pt]
HARP-Net
& domains $=3$;
latent dimension $\in \{32,64,96\}$;
temporal encoder $=\mathrm{GRU}$;
bridge steps $\in \{2,4\}$;
context layers $\in \{1,2,3\}$;
field layers $\in \{1,2,3\}$;
activation $\in \{\mathrm{GELU},\mathrm{ReLU},\mathrm{SiLU}\}$;
dropout $\in [0,0.15]$;
residual scale $\in \{0.05,0.10,0.25,0.50\}$;
prior correction scale $\in \{0.25,0.50,1.00\}$;
drift clip $\in \{0.02,0.05,0.10\}$
& learning rate $\in [5{\times}10^{-5},2{\times}10^{-3}]$;
batch paths $\in \{8,12,16,24\}$ \\

\end{longtable}
\noindent\scriptsize\raggedright
\textit{Note.}
Learning rates are sampled log-uniformly and
dropout rates uniformly over the specified
intervals. Batch paths denote the number of
complete option paths per optimization batch.
\par
\endgroup

==> tables/robustness.tex <==
\begin{table}[!htbp]
\centering
\caption{Robustness across random seeds for the main neural baselines.}
\label{tab:robustness-seed-pnl2}
\footnotesize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.12}
\begin{threeparttable}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Model} & \textbf{DJX Call} & \textbf{DJX Put} & \textbf{XEO Call} & \textbf{XEO Put} \\
\midrule
HARP-Net & \best{\shortstack{8.0579\\$\pm$ 0.4946}} & \best{\shortstack{9.1811\\$\pm$ 0.2521}} & \best{\shortstack{828.3690\\$\pm$ 39.7088}} & \best{\shortstack{1070.6956\\$\pm$ 12.8283}} \\
GRU & \shortstack{55.4906\\$\pm$ 22.5244} & \shortstack{42.2921\\$\pm$ 20.7488} & \shortstack{1407.8501\\$\pm$ 318.9742} & \shortstack{1491.2501\\$\pm$ 224.1459} \\
NLinear & \shortstack{75.9228\\$\pm$ 9.1388} & \shortstack{58.6058\\$\pm$ 15.8589} & \shortstack{2758.1223\\$\pm$ 791.3897} & \shortstack{2217.4424\\$\pm$ 551.1458} \\
PAttn & \shortstack{55.2659\\$\pm$ 5.3775} & \shortstack{54.5771\\$\pm$ 17.8131} & \shortstack{3072.2558\\$\pm$ 852.0036} & \shortstack{3135.0199\\$\pm$ 767.3476} \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\scriptsize\raggedright
\item \textit{Note.} Each entry reports the mean $\pm$ sample standard deviation of test hedging PnL$^2$ across seeds 40--44. Bold entries indicate the lowest mean for each task.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/statistical_summary.tex <==

\begin{table}[!htbp]
\centering
\caption{Summary of the Holm-adjusted Diebold--Mariano
tests and 95\% Model Confidence Sets.}
\label{tab:statistical_summary}

\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}

\begin{threeparttable}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule

& & \multicolumn{3}{c}{\textbf{DM rejections}}
& \multicolumn{3}{c}{\textbf{MCS size}} \\

\cmidrule(lr){3-5}
\cmidrule(lr){6-8}

\textbf{Dataset}
& $G$
& PnL$^2$
& $|\mathrm{Mean}|$
& Std
& PnL$^2$
& $|\mathrm{Mean}|$
& Std \\

\midrule

DJX-Call
& 9
& 0 & 5 & 16
& 12 & 10 & \textbf{1} \\

DJX-Put
& 9
& 0 & 4 & 18
& 12 & 6 & \textbf{1} \\

XEO-Call
& 40
& 3 & 11 & 13
& 9 & 2 & 4 \\

XEO-Put
& 41
& 3 & 7 & 15
& 12 & 11 & 4 \\

\midrule

\textbf{Total}
& --
& \textbf{6}
& \textbf{27}
& \textbf{62}
& -- & -- & -- \\

\bottomrule
\end{tabular}
\end{adjustbox}

\begin{tablenotes}[flushleft]
\scriptsize
\item \textit{Note.} $G$ denotes the number of
eligible expiration groups. DM rejections indicate
the number of pairwise comparisons favoring HARP-Net
at the Holm-adjusted 5\% significance level, out of
19 benchmarks per dataset and metric. MCS size
denotes the number of models retained in the 95\%
confidence set out of 20 candidate models.
HARP-Net is retained in all twelve confidence sets.
Bold MCS entries indicate that HARP-Net is the sole
retained model.
\end{tablenotes}

\end{threeparttable}
\end{table}

